Classification and Uncertainty Quantification of Corrupted Data using Semi-Supervised Autoencoders

Parametric and non-parametric classifiers often have to deal with real-world data, where corruptions like noise, occlusions, and blur are unavoidable - posing significant challenges. We present a probabilistic approach to classify strongly corrupted data and quantify uncertainty, despite the model only having been trained with uncorrupted data. A semi-supervised autoencoder trained on uncorrupted data is the underlying architecture. We use the decoding part as a generative model for realistic data and extend it by convolutions, masking, and additive Gaussian noise to describe imperfections. This constitutes a statistical inference task in terms of the optimal latent space activations of the underlying uncorrupted datum. We solve this problem approximately with Metric Gaussian Variational Inference (MGVI). The supervision of the autoencoder's latent space allows us to classify corrupted data directly under uncertainty with the statistically inferred latent space activations. Furthermore, we demonstrate that the model uncertainty strongly depends on whether the classification is correct or wrong, setting a basis for a statistical "lie detector" of the classification. Independent of that, we show that the generative model can optimally restore the uncorrupted datum by decoding the inferred latent space activations.

==> Definitions/journalnames.tex <==
%%Updated on 28 December 2021
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{Biomedinformatics}\gdef\@journalshort{Biomedinformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}\gdef\@continuouspages{yes}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{CTN}\gdef\@doiabbr{Clin. Transl. Neurosci.}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{currophthalmol}{\gdef\@journal{currophthalmol}\gdef\@journalfull{Current Ophthalmology}\gdef\@journalshort{Curr. Ophthalmol.}\gdef\@doiabbr{currophthalmol}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng-Advances in Engineering}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic. Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharm.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology Market and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kidneydial}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-coding RNA}\gdef\@journalshort{Non-coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{Synbio}\gdef\@journalshort{Synbio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}


==> images/figure1/FMNIST/classification.tex <==
% '''
% Data Corruption:

% 1. Mask --> Operator: M (no_mask, half_mask, corner_mask, checkerboard_mask, random_mask)
% 2. Noise --> Operator: N 
% 3. Convolution --> Operator: C (sobel, gaussian_blur, edge_detection, own)

% Data Modification (not included in modeling-process; thus the Model "does not 
% know" these modifications):

% 4. Rotation (angle)

% X. Response --> Operator: R (Concatenated Mask, Noise and Convolution)
% '''
% p=23
% #p = 10
% ground_truth = ift.Field.from_raw(position_space, np.reshape(XTest[p], position_space.shape))
% # 1. Mask
% #M = Mask.random_mask(n_blobs=25, seed=1, position_space=position_space)

% #M = Mask.no_mask(position_space=position_space)
% M = Mask.half_mask(position_space=position_space, mask_range=0.5)
% M = Mask.random_mask(position_space=position_space, seed=10, n_blobs=25)

% #M = Mask.half_mask(position_space=position_space, mask_range=0.5)
% # 2. Noise
% N, n = get_noise(noise_level=0.1, position_space=position_space, seed=10)

% # 3. Convolution
% C = Conv.gaussian_blur(5, 1, position_space=position_space) # sobel, edge_detection, 

% # 4. Rotation
% ground_truth_rot = rotation(ground_truth, img_shape, angle=0)

% # Apply Data Corruption to Ground Truth and creeate Response operator

% GR = ift.GeometryRemover(position_space)
% R = GR(M) # Without Convolution
% R = GR(M @ C) # With Convolution
% data = R((ground_truth_rot))+n# Apply Response R on (rotated) ground truth

% plt.imshow(np.reshape(data.val, img_shape))
% #plt.title('Corrupted Data')
% clear_axis()
% mpl.rcParams['figure.dpi']= 150
% mpl.rcParams['font.size'] = 9.0
% plt.show()
% print(np.mean(ground_truth.val))
\begin{tikzpicture} 
\begin{axis}[width=3.5cm, height=3.5cm,ymin=-8, ymax=13,bar width=3pt,
ticklabel style = {font=\tiny}, label style={font=\tiny}, minor xtick={0,1,2,3,4,5,6,7,8,9},xtick={0,1,2,3,4,5,6,7,8,9}]
    \addplot[fill=gray,
        ybar,
        error bars/.cd,
            y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt}
    ] coordinates {
(0, 0.9074392244183155)+-(0,1.2897490155704396)
(1, -4.977045835125597)+-(0,1.6892428130341155)
(3, -6.169149900227663)+-(0,1.4906571291241688)
(4, 7.0016367542685)+-(0,1.9787407434511237)
(5, 1.0576525645117487)+-(0,0.8607711571438896)
(6, 9.170315358639554)+-(0,1.9154243885163944)
(7, -5.311896177195083)+-(0,1.9562738457380366)
(8, -0.9274058253085375)+-(0,1.540772192430144)
(9, 0.24850070002522637)+-(0,1.2584509020932937)
};
    \addplot[fill=orange,
        ybar,
        error bars/.cd,
            y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt}
]
    coordinates{
(2, 9.843916010420887)+-(0,2.4146014584836357)
};
\addplot[fill=white,opacity=0.35,
	bar width=2pt,
        ybar,
       ] coordinates {
    (0, -0.12554067)
(1,  -6.1688843)
(2,  8.908215)
(3, -4.1438165 )
(4, 5.3111887)
(5,  -0.625254 )
(6,  7.619137)
(7,  -6.4036336 )
(8,  -2.3990023 )
(9,  -0.45938364)
};

\end{axis}
\end{tikzpicture}%
    ~%
    %
\begin{tikzpicture} 
\begin{axis}[width=3.5cm, height=3.5cm,ymin=-1, ymax=13,bar width=3pt,
ticklabel style = {font=\tiny},label style={font=\tiny}, minor xtick={0,1,2,3,4,5,6,7,8,9}, xtick={0,1,2,3,4,5,6,7,8,9}]
    \addplot[fill=gray,
        ybar,
        error bars/.cd,
            y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt}
    ] coordinates {
(0, 8.707195023162308)+-(0,1.4977375834377287)
(1, 9.176380978858075)+-(0,1.1452570537905868)
(2, 4.814811702723542)+-(0,1.1998797423448213)
(3, 6.930808346406654)+-(0,0.7820257299737633)
(5, 6.569816516811618)+-(0,0.8812136038399144)
(6, 5.045057432101427)+-(0,1.106191080862397)
(7, 10.058354320681083)+-(0,1.2246883856101713)
(8, 6.8303660543352045)+-(0,0.9496418695769726)
(9, 8.664000429789452)+-(0,1.4414580960060097)
    };
    \addplot[fill=orange,
        ybar,
        error bars/.cd,
            y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt}
]
    coordinates{
(4, 4.507322901808305)+-(0,0.9295378337849619)
};
\end{axis}
\end{tikzpicture}

==> images/figure1/MNIST/classification.tex <==
% '''
% Data Corruption:

% 1. Mask --> Operator: M (no_mask, half_mask, corner_mask, checkerboard_mask, random_mask)
% 2. Noise --> Operator: N 
% 3. Convolution --> Operator: C (sobel, gaussian_blur, edge_detection, own)

% Data Modification (not included in modeling-process; thus the Model "does not 
% know" these modifications):

% 4. Rotation (angle)

% X. Response --> Operator: R (Concatenated Mask, Noise and Convolution)
% '''
% p=23
% #p = 10
% ground_truth = ift.Field.from_raw(position_space, np.reshape(XTest[p], position_space.shape))
% # 1. Mask
% #M = Mask.random_mask(n_blobs=25, seed=1, position_space=position_space)

% #M = Mask.no_mask(position_space=position_space)
% M = Mask.half_mask(position_space=position_space, mask_range=0.5)
% M = Mask.random_mask(position_space=position_space, seed=10, n_blobs=25)

% #M = Mask.half_mask(position_space=position_space, mask_range=0.5)
% # 2. Noise
% N, n = get_noise(noise_level=0.1, position_space=position_space, seed=10)

% # 3. Convolution
% C = Conv.gaussian_blur(5, 1, position_space=position_space) # sobel, edge_detection, 

% # 4. Rotation
% ground_truth_rot = rotation(ground_truth, img_shape, angle=0)

% # Apply Data Corruption to Ground Truth and creeate Response operator

% GR = ift.GeometryRemover(position_space)
% R = GR(M) # Without Convolution
% R = GR(M @ C) # With Convolution
% data = R((ground_truth_rot))+n# Apply Response R on (rotated) ground truth

% plt.imshow(np.reshape(data.val, img_shape))
% #plt.title('Corrupted Data')
% clear_axis()
% mpl.rcParams['figure.dpi']= 150
% mpl.rcParams['font.size'] = 9.0
% plt.show()
% print(np.mean(ground_truth.val))

\begin{tikzpicture}

\begin{axis}[width=3.5cm, height=3.5cm,ymin=-6, ymax=7.5,align =center, title={\scriptsize{$\overline{\mathcal{H}}\pm\bm{\delta_r}$ \& $f(\bm{x})$}},bar width=3pt,
ticklabel style = {font=\tiny},label style={font=\tiny}, xmajorticks=false, minor xtick={0,1,2,3,4,5,6,7,8,9}]
    \addplot[fill=gray,
        ybar,
        error bars/.cd,
            y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt,}
    ] coordinates {
( 0 , -1.333790594849042 ) +- ( 0 , 0.3233276660861007 )
( 1 , -1.1111370552955604 ) +- ( 1 , 0.2225506278536135 )
( 2 , -0.9910260657828902 ) +- ( 2 , 0.41685151554656413 )
( 3 , -1.1539068430125368 ) +- ( 3 , 0.4447458254221104 )
( 5 , -0.29441899129954535 ) +- ( 5 , 0.37324412770211873 )
( 6 , -0.9489737369890273 ) +- ( 6 , 0.2104434266205051 )
( 7 , -0.18124802162347353 ) +- ( 7 , 0.5442769239194797 )
( 8 , 1.612331841522809 ) +- ( 8 , 0.8466116321569718 )
( 9 , -0.4826476718967445 ) +- ( 9 , 0.5321798306311084 )
};


    \addplot[fill=orange, ybar, error bars/.cd, y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt}]
    coordinates{
( 4 , 5.206786750464037 ) +- ( 4 , 1.7419255623674585 )
};
\addplot[fill=white,opacity=0.35,
	bar width=2pt,
        ybar,
       ] coordinates {
( 0 , -1.2548176 )
( 1 , -0.89296407 )
( 2 , -0.7592658 )
( 3 , -1.0203555 )
( 4 , 6.2007537 )
( 5 , -0.3555865 )
( 6 , -1.0464954 )
( 7 , -0.37164295 )
( 8 , 0.22147377 )
( 9 , -0.2920838 )
};
\end{axis}
\end{tikzpicture}
\begin{tikzpicture} 
\begin{axis}[width=3.5cm, height=3.5cm,ymin=-2, ymax=28, title={\scriptsize{$\bm{\delta_m} \pm \bm{\delta_r}$}},bar width=3pt,
ticklabel style = {font=\tiny},xmajorticks=false, minor xtick={0,1,2,3,4,5,6,7,8,9}]
    \addplot[fill=gray,
        ybar,
        error bars/.cd,
            y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt}
    ] coordinates {
( 0 , 20.060900428974247 ) +- ( 0 , 2.481000554583958 )
( 1 , 20.302899200116165 ) +- ( 1 , 3.931952257097683 )
( 2 , 13.478442920276086 ) +- ( 2 , 2.4467014087870234 )
( 3 , 16.663533187713163 ) +- ( 3 , 3.3978423168627865 )
( 5 , 15.009544905231017 ) +- ( 5 , 2.847201424411398 )
( 6 , 21.421548279312482 ) +- ( 6 , 4.588945759841051 )
( 7 , 17.030865720530574 ) +- ( 7 , 3.5992408442589046 )
( 8 , 15.150060199892284 ) +- ( 8 , 3.5013285936482794 )
( 9 , 12.692934176045009 ) +- ( 9 , 2.425891296322672 )
    };
    \addplot[fill=orange, ybar, error bars/.cd, y dir=both, y explicit,
            error bar style={line width=0.75pt},
    error mark options={
      mark size=0pt,
      rotate=90,
      line width=0.5pt}]
    coordinates{
( 4 , 5.288998946438056 ) +- ( 4 , 1.1408347018587885 )
};
\end{axis}
\end{tikzpicture}

==> images/figure1/pipeline.tex <==
% This file loads all images to build figure1, from both the MNIST-File and the FMNIST-file. 

\begin{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MNIST (Top row)

\node(0){\includegraphics[scale=0.25]{images/figure1/MNIST/mnist_gt.png}};
\node[right=0.25cm of 0](1){\includegraphics[scale=0.25]{images/figure1/MNIST/mnist_data.png}};
\node[xshift=2.5cm, yshift=0.4cm](bars1) at (1.east) {\input{images/figure1/MNIST/classification.tex}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fashion-MNIST (Bottom row)

\node[below=0.1cm of 0](0a){\includegraphics[scale=0.25]{images/figure1/FMNIST/fashion_mnist_ground_truth.png}};
\node[right=0.25cm of 0a](1a){\includegraphics[scale=0.25]{images/figure1/FMNIST/fashion_mnist_data.png}};
\node[xshift=2.5cm, yshift=-0.15cm](bars2)at (1a.east){\input{images/figure1/FMNIST/classification.tex}};
  % curly brace
  \begin{scope}[shift={(3,0)}]
  \draw[decorate, decoration={brace, amplitude=1ex, raise=1ex}](1.2, 1.6) -- (5.8, 1.6) node[pos=.5, above=2.5ex, align=center] {\scriptsize{\textsc{Latent-Space}:}\\ \scriptsize{Classification and Uncertainty Quantification}};
    \end{scope}
\node[right=0.25cm of bars1, yshift=-0.4cm](2){\includegraphics[scale=0.25]{images/figure1/MNIST/mnist_decoded_posterior_mean.png}};
\node[above=0.05cm of 2, text width=3cm, align=center](2a){\scriptsize{\textsc{Reconstruction}\\$g(\overline{\mathcal{H}})$}};
\node[right=0.19cm of bars2, yshift=0.15cm](2a){\includegraphics[scale=0.25]{images/figure1/FMNIST/fmnist_posterior_mean_decoded.png}};
\node[above=0.05cm of 0, text width=3cm, align=center](0a){\scriptsize{\textsc{Ground-Truth}\\ $\vphantom{\bm{mC}}\bm{x}$}};
\node[above=0.05cm of 1, text width=3cm, align=center](1a){\scriptsize{\textsc{Corrupted Datum}\\ $\bm{d}=\bm{mC}\bm{x}+\bm{n}$}};
\end{tikzpicture}


==> images/figure10/convolution_fmnist.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[baseline, scale=0.75]
\begin{axis}[scale=0.75,axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.1, xmax=10,
            xmode=log,
            xmajorgrids,
            xminorgrids,
            	title=\Large{(3)},
            xlabel=Convolution level $\gamma$,
            ylabel=$\mathrm{ACC}^h$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.5, transform shape}}]
\addplot[black, mark=o] coordinates {
(0.1, 0.724)
(0.2, 0.737)
(0.3, 0.74)
(0.4, 0.734)
(0.5, 0.726)
(0.6, 0.715)
(0.7, 0.725)
(0.8, 0.706)
(0.9, 0.698)
(1, 0.678)
(1.1, 0.667)
(1.2, 0.657)
(1.3, 0.655)
(1.4, 0.629)
(1.5, 0.611)
(1.6, 0.63)
(1.7, 0.627)
(1.8, 0.616)
(1.9, 0.62)
(2, 0.605)
(3, 0.59)
(4, 0.593)
(5, 0.588)
(6, 0.605)
(7, 0.595)
(8, 0.598)
(9, 0.589)
(10, 0.596)
    };
\addplot[gray, mark=diamond] coordinates {
(0.1, 0.249)
(0.2, 0.249)
(0.3, 0.249)
(0.4, 0.249)
(0.5, 0.248)
(0.6, 0.252)
(0.7, 0.254)
(0.8, 0.256)
(0.9, 0.254)
(1, 0.263)
(1.1, 0.266)
(1.2, 0.266)
(1.3, 0.263)
(1.4, 0.258)
(1.5, 0.254)
(1.6, 0.253)
(1.7, 0.258)
(1.8, 0.258)
(1.9, 0.255)
(2, 0.254)
(3, 0.265)
(4, 0.266)
(5, 0.266)
(6, 0.263)
(7, 0.262)
(8, 0.264)
(9, 0.263)
(10, 0.264)
};
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0.1,0.1)
(10,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.75,axis y line*=right,
            ymin=0, ymax=2,
            xmin=0.1, xmax=10,
            axis x line=none,
            xmode=log,
            ylabel=\textcolor{red}{$\delta_r$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.05,0.4)},anchor=west},
            legend style={nodes={scale=0.5, transform shape}}]


\addplot[red, mark=x] coordinates {
(0.1, 0.7520151136052432)
(0.2, 0.7631758607683086)
(0.3, 0.7598074006148909)
(0.4, 0.8033684914166007)
(0.5, 0.8246240522606939)
(0.6, 0.883297859326738)
(0.7, 0.9270637519292175)
(0.8, 0.9723103747959162)
(0.9, 1.0128363797850595)
(1, 1.0510415281026462)
(1.1, 1.0772859397056613)
(1.2, 1.1096595100919449)
(1.3, 1.1425562018394442)
(1.4, 1.15807875707194)
(1.5, 1.186276737831649)
(1.6, 1.2056408972071306)
(1.7, 1.2178566519280802)
(1.8, 1.234282360072434)
(1.9, 1.25016362817768)
(2, 1.2528493169773356)
(3, 1.2988096767746238)
(4, 1.3154049173153726)
(5, 1.3182327475968154)
(6, 1.3149221490271477)
(7, 1.3175588118341082)
(8, 1.32280561094349)
(9, 1.3194298190280196)
(10, 1.3221662187065544)
    };
    \addplot[orange, mark=|] coordinates {
   (0.1, 0.7520151136052432)
(0.2, 0.7631758607683086)
(0.3, 0.7598074006148909)
(0.4, 0.8033684914166007) 
(0.5, 0.8726737838450338)
(0.6, 0.9362124139134462)
(0.7, 0.9699268165305917)
(0.8, 1.0157436902348738)
(0.9, 1.0629435344037963)
(1, 1.10083461077639)
(1.1, 1.1318872433939808)
(1.2, 1.1607021974654936)
(1.3, 1.197711646698145)
(1.4, 1.2205796893695293)
(1.5, 1.24190566877145)
(1.6, 1.2484384380504225)
(1.7, 1.2606953532722318)
(1.8, 1.285003432808937)
(1.9, 1.289135044733092)
(2, 1.2834933073784256)
(3, 1.3326393104692698)
(4, 1.355519585903645)
(5, 1.351594856432054)
(6, 1.3510409012064921)
(7, 1.3605745503899787)
(8, 1.3624059813108624)
(9, 1.359782241514213)
(10, 1.364997452091469)
    };
\addplot[orange, mark=-] coordinates {
(0.1, 0.7194613680426747)
(0.2, 0.7132908970387413)
(0.3, 0.7211049623467323)
(0.4, 0.7495600499379927)
(0.5, 0.8064895805608191)
(0.6, 0.8622060438621061)
(0.7, 0.9108053481149032)
(0.8, 0.954223413409155)
(0.9, 0.991156779935692)
(1, 1.027393485888862)
(1.1, 1.0500262183740119)
(1.2, 1.0830116535179306)
(1.3, 1.113504860654327)
(1.4, 1.1212141372270976)
(1.5, 1.1508599552856873)
(1.6, 1.1805058335372607)
(1.7, 1.1923720656420063)
(1.8, 1.2026640290159125)
(1.9, 1.226277921256621)
(2, 1.2328420835749712)
(3, 1.2753009482749542)
(4, 1.2878725899706394)
(5, 1.2948565761000157)
(6, 1.2913404843811296)
(7, 1.288279191472549)
(8, 1.2961846261814773)
(9, 1.2912721863593855)
(10, 1.2931329665463103)

    };

  \end{axis}
\end{tikzpicture}
\begin{tikzpicture}[baseline, scale=0.75]
\begin{axis}[scale=0.75,axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.1, xmax=10,
            	xmode=log,
            xmajorgrids,
            xminorgrids,
            xlabel=Convolution level $\gamma$,
            ylabel=$\mathrm{ACC}^{\delta_m}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.5, transform shape}},]

            
            
\addplot[black, mark=o] coordinates {
(0.1, 0.527)
(0.2, 0.539)
(0.3, 0.538)
(0.4, 0.539)
(0.5, 0.506)
(0.6, 0.483)
(0.7, 0.45)
(0.8, 0.435)
(0.9, 0.404)
(1, 0.369)
(1.1, 0.368)
(1.2, 0.334)
(1.3, 0.321)
(1.4, 0.295)
(1.5, 0.298)
(1.6, 0.291)
(1.7, 0.288)
(1.8, 0.285)
(1.9, 0.267)
(2, 0.282)
(3, 0.269)
(4, 0.256)
(5, 0.271)
(6, 0.272)
(7, 0.265)
(8, 0.257)
(9, 0.27)
(10, 0.278)
    };
\addplot[gray, mark=diamond] coordinates {
(0.1, 0.206)
(0.2, 0.206)
(0.3, 0.206)
(0.4, 0.212)
(0.5, 0.21)
(0.6, 0.22)
(0.7, 0.228)
(0.8, 0.23)
(0.9, 0.235)
(1, 0.237)
(1.1, 0.242)
(1.2, 0.244)
(1.3, 0.242)
(1.4, 0.24)
(1.5, 0.239)
(1.6, 0.24)
(1.7, 0.238)
(1.8, 0.236)
(1.9, 0.236)
(2, 0.237)
(3, 0.242)
(4, 0.244)
(5, 0.244)
(6, 0.244)
(7, 0.243)
(8, 0.243)
(9, 0.242)
(10, 0.242)
    };
    \addplot[gray,smooth, mark=none, dashed] coordinates {
(0.1,0.1)
(10,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.75,axis y line*=right,
            ymin=6, ymax=15,
            xmin=0.1, xmax=10,
            xmode=log,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_m$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.01,0.4)},anchor=west},
            legend style={nodes={scale=0.5, transform shape}},]

\addplot[red, mark=x] coordinates {
(0.1, 8.540919745500032)
(0.2, 8.4423886349936)
(0.3, 8.507186246537549)
(0.4, 8.630645347539907)
(0.5, 9.153874717209927)
(0.6, 9.412250514607617)
(0.7, 9.712787978944673)
(0.8, 10.056266427020525)
(0.9, 10.249406480736813)
(1, 10.615232536405323)
(1.1, 10.787716429325567)
(1.2, 11.02622029052355)
(1.3, 11.362826570749348)
(1.4, 11.39597412900349)
(1.5, 11.697360160752714)
(1.6, 11.766366294577063)
(1.7, 11.863735125224773)
(1.8, 12.06597152109904)
(1.9, 12.141444238653362)
(2, 12.112043730725185)
(3, 12.480090230585896)
(4, 12.522726547443847)
(5, 12.525195888185845)
(6, 12.57065103783848)
(7, 12.510161168634099)
(8, 12.534147678215337)
(9, 12.54970080461622)
(10, 12.536281242105344)
    };
\addplot[orange, mark=|] coordinates {
(0.1, 11.034735282575843)
(0.2, 10.970262700821525)
(0.3, 10.973283000771213)
(0.4, 11.15018405783686)
(0.5, 11.65480943416844)
(0.6, 11.745016691104777)
(0.7, 11.890039238756275)
(0.8, 12.22905050596786)
(0.9, 12.209505592680733)
(1, 12.48359238332134)
(1.1, 12.77738425904627)
(1.2, 12.821992097169073)
(1.3, 13.224908502193447)
(1.4, 13.017109596441216)
(1.5, 13.387965371557295)
(1.6, 13.386874746591138)
(1.7, 13.475130196178482)
(1.8, 13.670425202280208)
(1.9, 13.596834788999438)
(2, 13.683239526058706)
(3, 13.972852017781234)
(4, 13.828195653518383)
(5, 13.922746922575175)
(6, 14.035177914982727)
(7, 13.944619362708167)
(8, 13.787039927742782)
(9, 13.906276017423417)
(10, 13.953186030277095)
    };
\addplot[orange, mark=-] coordinates {
(0.1, 6.302637489263109)
(0.2, 6.280329369044299)
(0.3, 6.389460037511615)
(0.4, 6.475715207564218)
(0.5, 6.712250705001417)
(0.6, 6.915273054464691)
(0.7, 7.0517031058416055)
(0.8, 7.234144577353293)
(0.9, 7.35777511757202)
(1, 7.420286565120752)
(1.1, 7.370678200022619)
(1.2, 7.445429801823195)
(1.3, 7.424030211090336)
(1.4, 7.521735130550618)
(1.5, 7.714793523219779)
(1.6, 7.818117179532459)
(1.7, 7.880008422033659)
(1.8, 8.040763163048041)
(1.9, 8.145933851373684)
(2, 8.11162323054977)
(3, 8.423551693634995)
(4, 8.728706957914724)
(5, 8.765732035529677)
(6, 8.650887925481827)
(7, 8.53156957374942)
(8, 8.911972808958947)
(9, 8.881923377396765)
(10, 8.856406216709644)
    };


  \end{axis}
\end{tikzpicture}

==> images/figure10/noise_acc_sae_fmnist.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[baseline, scale=0.75]
\begin{axis}[scale=0.75,
xmode=log,
            log ticks with fixed point,
            axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.01, xmax=10,
            xmajorgrids,
            xminorgrids,
            	title=\Large{(1)},
            xlabel=Noise level $\alpha$,
            ylabel=$\mathrm{ACC}^{h}$,every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},]
\addplot[black, mark=o] coordinates {
(0.01, 0.775)
(0.02, 0.778)
(0.03, 0.784)
(0.04, 0.785)
(0.05, 0.794)
(0.06, 0.796)
(0.07, 0.788)
(0.08, 0.791)
(0.09, 0.79)
(0.1, 0.783)
(0.2, 0.768)
(0.3, 0.741)
(0.4, 0.728)
(0.5, 0.717)
(0.6, 0.709)
(0.7, 0.686)
(0.8, 0.681)
(0.9, 0.665)
(1, 0.653)
(2, 0.525)
(3, 0.462)
(4, 0.401)
(5, 0.356)
(6, 0.314)
(7, 0.283)
(8, 0.246)
(9, 0.242)
(10, 0.223)
    };
  \label{plot_one_top_2}

    \addplot[gray, mark=diamond] coordinates {   
(0.01, 0.884)
(0.02, 0.863)
(0.03, 0.852)
(0.04, 0.834)
(0.05, 0.824)
(0.06, 0.809)
(0.07, 0.789)
(0.08, 0.767)
(0.09, 0.748)
(0.1, 0.728)
(0.2, 0.562)
(0.3, 0.408)
(0.4, 0.317)
(0.5, 0.28)
(0.6, 0.269)
(0.7, 0.239)
(0.8, 0.225)
(0.9, 0.207)
(1, 0.192)
(2, 0.118)
(3, 0.095)
(4, 0.095)
(5, 0.095)
(6, 0.095)
(7, 0.095)
(8, 0.095)
(9, 0.095)
(10, 0.095)
};
\label{plot_one_b}
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0.01,0.1)
(10,0.1)
    };
\label{Random_top_2}
\end{axis}  
\begin{axis}[scale=0.75,xmode=log,
            log ticks with fixed point,
            axis y line*=right,
            ymin=0, ymax=2,
            xmin=0.01, xmax=10,
            axis x line=none,
            ylabel=\textcolor{red}{${\delta}_r$},every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(-0.8,0.5)},anchor=west},
            legend style={nodes={scale=0.9, transform shape}}]
                        \addlegendimage{mark=o}
\addlegendentry{$\mathrm{ACC}_g$}

\addlegendimage{mark=diamond, gray}
\addlegendentry{$\mathrm{ACC}_f$}
\addlegendimage{mark=none, gray, dashed}
\addlegendentry{Random}
\addplot[red, mark=x] coordinates {
(0.01, 0.25689617419785915)
(0.02, 0.35346797363346144)
(0.03, 0.42147238703129636)
(0.04, 0.47265288834919944)
(0.05, 0.5198574760523398)
(0.06, 0.5583837359655169)
(0.07, 0.5921107997299986)
(0.08, 0.6178314140816046)
(0.09, 0.6482904000758066)
(0.1, 0.6737680100964161)
(0.2, 0.8488522219088417)
(0.3, 0.9531938096575782)
(0.4, 1.0204896179416578)
(0.5, 1.0739780724470138)
(0.6, 1.1137049825363388)
(0.7, 1.1459984140339998)
(0.8, 1.1785206548403635)
(0.9, 1.202030204790946)
(1, 1.2226064596336332)
(2, 1.358338343511709)
(3, 1.4426208985859021)
(4, 1.5032579958760455)
(5, 1.5391342999407496)
(6, 1.57867910897211)
(7, 1.6060053009210484)
(8, 1.630490079190739)
(9, 1.6476339777779183)
(10, 1.671059806541454)
    };

    \addplot[orange, mark=|] coordinates {
(0.01, 0.2689854925495836)
(0.02, 0.3760531418328386)
(0.03, 0.4544636745828688)
(0.04, 0.4884267424985628)
(0.05, 0.5470448667834767)
(0.06, 0.5954530770951896)
(0.07, 0.6203347617932621)
(0.08, 0.6493013693071171)
(0.09, 0.6782173777789687)
(0.1, 0.7054895244483198)
(0.2, 0.8843970571802505)
(0.3, 0.9909469132779769)
(0.4, 1.0727393301350592)
(0.5, 1.1238904835434997)
(0.6, 1.1727463317689997)
(0.7, 1.205401675644642)
(0.8, 1.2390701418010395)
(0.9, 1.254501283057492)
(1, 1.2655349804476632)
(2, 1.3803811592566892)
(3, 1.463145937609717)
(4, 1.5182652997948274)
(5, 1.5517519626145133)
(6, 1.5895587841405838)
(7, 1.6144013561186392)
(8, 1.6348030417439852)
(9, 1.6518375241297505)
(10, 1.674118953255155)
    };
\label{std_false_top_2}
\addplot[orange, mark=-] coordinates {
(0.01, 0.25338637209574555)
(0.02, 0.34702336265626127)
(0.03, 0.4123829506650468)
(0.04, 0.4683326607796286)
(0.05, 0.512803820522599)
(0.06, 0.5488835530629376)
(0.07, 0.58451755105308)
(0.08, 0.6095163437375691)
(0.09, 0.6403351275218014)
(0.1, 0.6649767347268591)
(0.2, 0.8381147195872702)
(0.3, 0.9399980554906642)
(0.4, 1.0009677474518155)
(0.5, 1.0542776368259463)
(0.6, 1.0894722143745554)
(0.7, 1.1188079998273794)
(0.8, 1.15015753246084)
(0.9, 1.1755974059649412)
(1, 1.1997945197829925)
(2, 1.3383948435519648)
(3, 1.4187194462161783)
(4, 1.4808406017430022)
(5, 1.5163090899354015)
(6, 1.5549101371072274)
(7, 1.5847333165511808)
(8, 1.617270673641359)
(9, 1.6344674978825098)
(10, 1.660400806556944)
    };
\label{std_true_top_2}

\addlegendimage{/pgfplots/refstyle=plot_one_top_2}\addlegendentry{${\delta}_r$}
\addlegendimage{/pgfplots/refstyle=std_true_top_2}\addlegendentry{${\delta}_{r_{\mathrm{False}}}$}
\addlegendimage{/pgfplots/refstyle=std_false_top_2}\addlegendentry{${\delta}_{r_{\mathrm{True}}}$}

  \end{axis}
\end{tikzpicture}\\
\begin{tikzpicture}[baseline, scale=0.75]
\begin{axis}[scale=0.75,xmode=log,
            log ticks with fixed point,
            axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.01, xmax=10,
            xmajorgrids,
            xminorgrids,
            xlabel=Noise level $\alpha$,
            ylabel=$\mathrm{ACC}^{\delta_m}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
}]
\addplot[black, mark=o] coordinates {
(0.01, 0.691)
(0.02, 0.697)
(0.03, 0.709)
(0.04, 0.692)
(0.05, 0.69)
(0.06, 0.689)
(0.07, 0.677)
(0.08, 0.681)
(0.09, 0.669)
(0.1, 0.656)
(0.2, 0.588)
(0.3, 0.523)
(0.4, 0.47)
(0.5, 0.435)
(0.6, 0.407)
(0.7, 0.379)
(0.8, 0.359)
(0.9, 0.324)
(1, 0.292)
(2, 0.197)
(3, 0.153)
(4, 0.146)
(5, 0.128)
(6, 0.119)
(7, 0.12)
(8, 0.113)
(9, 0.106)
(10, 0.108)
    };


\label{plot_one_bottom_2}
\addplot[gray, mark=diamond] coordinates {
(0.01, 0.877)
(0.02, 0.864)
(0.03, 0.843)
(0.04, 0.823)
(0.05, 0.796)
(0.06, 0.778)
(0.07, 0.761)
(0.08, 0.732)
(0.09, 0.707)
(0.1, 0.684)
(0.2, 0.489)
(0.3, 0.357)
(0.4, 0.279)
(0.5, 0.244)
(0.6, 0.219)
(0.7, 0.186)
(0.8, 0.158)
(0.9, 0.139)
(1, 0.129)
(2, 0.106)
(3, 0.115)
(4, 0.115)
(5, 0.115)
(6, 0.115)
(7, 0.115)
(8, 0.115)
(9, 0.115)
(10, 0.115)
    };
\label{plot_two_b}
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0.01,0.1)
(10,0.1)
    };
\label{Random_bottom_2}
\end{axis}  
\begin{axis}[scale=0.75,xmode=log,
            log ticks with fixed point,
            axis y line*=right,
            ymin=3, ymax=14,
            xmin=0.01, xmax=10,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_m$},every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(-0.8,0.5)},anchor=west},
            legend style={nodes={scale=0.9, transform shape}}]
                        \addlegendimage{mark=o}
\addlegendentry{$\mathrm{ACC}_g$}

\addlegendimage{mark=diamond, gray}
\addlegendentry{$\mathrm{ACC}_f$}
\addlegendimage{mark=none, gray, dashed}
\addlegendentry{Random}
\addplot[red, mark=x] coordinates {
(0.01, 6.855687145838454)
(0.02, 6.8119625841499785)
(0.03, 6.8791810407723055)
(0.04, 6.990196551689949)
(0.05, 7.121383840186811)
(0.06, 7.185194943114889)
(0.07, 7.350022051379889)
(0.08, 7.392263526293117)
(0.09, 7.545537522501774)
(0.1, 7.684064854238299)
(0.2, 8.465089418642286)
(0.3, 8.901601213893315)
(0.4, 9.16834988517917)
(0.5, 9.415235390027734)
(0.6, 9.564138609464305)
(0.7, 9.694972493678703)
(0.8, 9.816517777990354)
(0.9, 9.90232604199593)
(1, 10.035704990239843)
(2, 10.63065693250225)
(3, 11.008702904038971)
(4, 11.263617685733063)
(5, 11.355309347959478)
(6, 11.536409373989267)
(7, 11.631846739387024)
(8, 11.739618114436693)
(9, 11.761930140542816)
(10, 11.85082358881609)
    };
\addplot[orange, mark=|] coordinates {
(0.01, 10.925015745943467)
(0.02, 10.54668191298834)
(0.03, 10.451803415184141)
(0.04, 10.349454939196985)
(0.05, 10.452696767475258)
(0.06, 10.40795661806871)
(0.07, 10.422508624235844)
(0.08, 10.433023879092328)
(0.09, 10.460723639517658)
(0.1, 10.58601685874351)
(0.2, 10.822063839062833)
(0.3, 10.767801701607127)
(0.4, 10.725706880109534)
(0.5, 10.908862259013047)
(0.6, 10.87860743928997)
(0.7, 10.903310751967116)
(0.8, 10.932675335845696)
(0.9, 10.834800075580857)
(1, 10.902087915670545)
(2, 11.188518788434804)
(3, 11.44615500905555)
(4, 11.696029379349167)
(5, 11.747956084617718)
(6, 11.896697090375573)
(7, 12.00018848358307)
(8, 12.08974050468684)
(9, 12.09657460852456)
(10, 12.186071056506702)
    };
\label{std_false_bottom_2}
\addplot[orange, mark=-] coordinates {
(0.01, 5.035972909322609)
(0.02, 5.188404540192985)
(0.03, 5.4128437897795765)
(0.04, 5.4950353040712105)
(0.05, 5.624707017781855)
(0.06, 5.7305086137815975)
(0.07, 5.884123730800165)
(0.08, 5.967883860297598)
(0.09, 6.103195811392271)
(0.1, 6.162309534802639)
(0.2, 6.813603940388433)
(0.3, 7.199540730835019)
(0.4, 7.4121813589810985)
(0.5, 7.475237272839912)
(0.6, 7.648954294755163)
(0.7, 7.715083157538586)
(0.8, 7.82360135853276)
(0.9, 7.956793799084174)
(1, 7.935023102551701)
(2, 8.356732717711179)
(3, 8.586990923979876)
(4, 8.734305450471735)
(5, 8.680403454475233)
(6, 8.869069221583091)
(7, 8.930673948616011)
(8, 8.991312272384636)
(9, 8.939551325677922)
(10, 9.081927837149168)
    };
\label{std_true_bottom_2}
\addlegendimage{/pgfplots/refstyle=plot_one_bottom_2}\addlegendentry{$\delta_m$}
\addlegendimage{/pgfplots/refstyle=std_false_bottom_2}\addlegendentry{$\delta_{m_{\mathrm{False}}}$}
\addlegendimage{/pgfplots/refstyle=std_true_bottom_2}\addlegendentry{$\delta_{m_{\mathrm{True}}}$}

  \end{axis}
\end{tikzpicture}


==> images/figure10/window_mask_acc_sae_fmnist.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[baseline, scale=0.75]
\begin{axis}[scale=0.75,axis y line*=left,
            ymin=0, ymax=1,
            xmin=1, xmax=14,
            xmajorgrids,
            xminorgrids,
            title=\Large{(2)},
            xlabel=Masking level $\beta$,
            ylabel=$\mathrm{ACC}^{h}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.75, transform shape}}]
\addplot[black, mark=o] coordinates {
(0, 0.783)
(1, 0.775)
(2, 0.746)
(3, 0.699)
(4, 0.637)
(5, 0.592)
(6, 0.559)
(7, 0.462)
(8, 0.321)
(9, 0.295)
(10, 0.335)
(11, 0.291)
(12, 0.235)
(13, 0.18)
(14, 0.097)
    };

\addplot[gray, mark=diamond] coordinates {
(0, 0.728)
(1, 0.661)
(2, 0.512)
(3, 0.423)
(4, 0.309)
(5, 0.283)
(6, 0.243)
(7, 0.134)
(8, 0.095)
(9, 0.095)
(10, 0.095)
(11, 0.095)
(12, 0.095)
(13, 0.095)
(14, 0.095)
};
\addplot[gray,smooth, mark=none, dashed] coordinates {
(1,0.1)
(14,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.75,axis y line*=right,
            ymin=0, ymax=2.5,
            xmin=1, xmax=14,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_r$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.05,0.4)},anchor=west},
            legend style={nodes={scale=0.75, transform shape}}]

\addplot[red, mark=x] coordinates {
(0, 0.6737680100964161)
(1, 0.7057749699979622)
(2, 0.7489427302641237)
(3, 0.8083413083790432)
(4, 0.9437209819457657)
(5, 0.944185544547026)
(6, 1.0015097625333107)
(7, 1.1378684843064966)
(8, 1.2426667820412145)
(9, 1.4390589970544951)
(10, 1.6335094815688467)
(11, 1.7605901040136855)
(12, 1.8037527521267156)
(13, 1.968236528975981)
(14, 2.1693131386327065)
    };

    \addplot[orange, mark=|] coordinates {
    (0, 0.7054895244483198)
(1, 0.7328048624014242)
(2, 0.7863219872336135)
(3, 0.8426991982919149)
(4, 1.0740376598979833)
(5, 0.972254365852653)
(6, 1.0309092223491103)
(7, 1.1874033994473978)
(8, 1.274911714625169)
(9, 1.4643272069754567)
(10, 1.6584018540611327)
(11, 1.7559876677393207)
(12, 1.7867807518158252)
(13, 1.9612821274332661)
(14, 2.16779189300034)
    };
\addplot[orange, mark=-] coordinates {
(0, 0.6649767347268591)
(1, 0.697927581880828)
(2, 0.7362157446471661)
(3, 0.7935462799616264)
(4, 0.8694588876025084)
(5, 0.9248408163499047)
(6, 0.9783162709791648)
(7, 1.0801849684064861)
(8, 1.1744602112483638)
(9, 1.378672258090841)
(10, 1.584096264531921)
(11, 1.7718035999536321)
(12, 1.8590020297345073)
(13, 1.9999176915594594)
(14, 2.183474837663909)
    };
  \end{axis}
\end{tikzpicture}\\
\begin{tikzpicture}[baseline, scale=0.75]
\begin{axis}[scale=0.75,axis y line*=left,
            ymin=0, ymax=1,
            xmin=1, xmax=14,
            xmajorgrids,
            xminorgrids,
            xlabel=Masking level $\beta$,
            ylabel=$\mathrm{ACC}^{\delta_m}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.75, transform shape}},]

            
            
\addplot[black, mark=o] coordinates {
(0, 0.656)
(1, 0.658)
(2, 0.592)
(3, 0.541)
(4, 0.462)
(5, 0.401)
(6, 0.355)
(7, 0.293)
(8, 0.206)
(9, 0.179)
(10, 0.145)
(11, 0.119)
(12, 0.101)
(13, 0.096)
(14, 0.097)
    };
\addplot[gray, mark=diamond] coordinates {
(0, 0.684)
(1, 0.613)
(2, 0.426)
(3, 0.349)
(4, 0.256)
(5, 0.228)
(6, 0.142)
(7, 0.123)
(8, 0.115)
(9, 0.115)
(10, 0.115)
(11, 0.115)
(12, 0.115)
(13, 0.115)
(14, 0.115)
    };
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0,0.1)
(14,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.75,axis y line*=right,
            ymin=3, ymax=17.5,
            xmin=1, xmax=14,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_m$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.01,0.4)},anchor=west},
            legend style={nodes={scale=0.75, transform shape}},]
\addplot[red, mark=x] coordinates {
(0, 7.684064854238299)
(1, 7.882109967580531)
(2, 8.418488969564136)
(3, 9.08727259697828)
(4, 9.904620430634596)
(5, 11.130726837716034)
(6, 11.359112486779948)
(7, 11.989800520385627)
(8, 13.035068950871542)
(9, 13.468589288420384)
(10, 13.483076271012422)
(11, 13.540669647643412)
(12, 12.877177244333328)
(13, 13.059621055025133)
(14, 13.63565466407137)
    };

\addplot[orange, mark=|] coordinates {
(0, 10.58601685874351)
(1, 10.744085967111864)
(2, 11.137565908083516)
(3, 11.621953905617714)
(4, 12.231235921360527)
(5, 13.756256134796358)
(6, 13.289816238002237)
(7, 13.445119318758021)
(8, 14.043600402544426)
(9, 14.319553320372222)
(10, 14.184573269672034)
(11, 14.108263847984423)
(12, 13.379916172211795)
(13, 13.569204344426844)
(14, 14.159720059944592)
    };

\addplot[orange, mark=-] coordinates {
(0, 6.162309534802639)
(1, 6.394578369039929)
(2, 6.544530538962943)
(3, 6.93677588595148)
(4, 7.195271655719983)
(5, 7.208801528611012)
(6, 7.851214121883114)
(7, 8.478160962538247)
(8, 9.147816656559556)
(9, 9.56556431505469)
(10, 9.346662934088503)
(11, 9.338564685454905)
(12, 8.40230302490026)
(13, 8.261045079825685)
(14, 8.75698402001448)
    };
\end{axis}

\end{tikzpicture}

==> images/figure2/steps.tex <==
  \begin{tikzpicture}[scale=0.6]
  \draw[ultra thick, color=gray] (0, 0) -- (0, 3.92);
    \draw[dashed, -latex, color=gray] (0, 3.92) --(1, 3.2);
    \draw[dashed, -latex, color=gray] (0, 0) --(1,0.64);
    \node at (0, 4.5) {\textcolor{gray}{\tiny{$[784]$}}};
    \node at (-0.2, 1.96) (x) {\textcolor{gray}{\tiny{$\bm{x}$}}};
    
    \draw[ultra thick, color=gray] (1,0.64) -- (1,3.2);
    \draw[dashed, -latex, color=gray] (1,3.2) --(2, 2.6);
    \draw[dashed, -latex, color=gray] (1,0.64) --(2,1.32);
    \node at (1, 4.0) {\textcolor{gray}{\tiny{$[512]$}}};
    
    \draw[ultra thick, color=gray] (2,1.32) -- (2, 2.6);
    \draw[dashed, -latex, color=gray] (2,2.6) --(3, 2.28);
    \draw[dashed, -latex, color=gray] (2,1.32) --(3,1.64);
    \node at (2, 3.5) {\textcolor{gray}{\tiny{$[256]$}}};
    
    \draw[ultra thick, color=gray](3, 1.64) -- (3, 2.28);
    \draw[dashed, -latex, color=gray] (3,2.28) --(4, 1.9858);
    \draw[dashed, -latex, color=gray] (3,1.64) --(4,1.935);
    \node at (3, 3.2) {\textcolor{gray}{\tiny{$[128]$}}};
    
    \draw[ultra thick] (4,1.935) -- (4,1.985);
    \draw[dashed, -latex] (4,1.985) --(5, 2.28);
    \draw[dashed, -latex] (4,1.935) --(5,1.64);
    \node at (4, 3.0) {\tiny{$[10]$}};
    \node at (4, 1.6) {\tiny{$\bm{h}$}};
    
    \draw[ultra thick] (5,1.64) -- (5,2.28);
    \draw[dashed, -latex] (5,2.28) --(6, 2.6);
    \draw[dashed, -latex] (5,1.64) --(6,1.32);
    \node at (5, 3.2) {\tiny{$[128]$}};    
        
    \draw[ultra thick] (6,1.32) -- (6, 2.6);
    \draw[dashed, -latex] (6,2.6) --(7, 3.2);
    \draw[dashed, -latex] (6,1.32) --(7,0.64);
    \node at (6, 3.5) {\tiny{$[256]$}};    
        
    \draw[ultra thick](7, 0.64) -- (7, 3.2);
    \draw[dashed, -latex] (7,3.2) --(8, 3.92);
    \draw[dashed, -latex] (7,0.64) --(8,0);
    \node at (7, 4.0) {\tiny{$[512]$}};    
    
    \draw[ultra thick] (8,0) -- (8,3.92);
    \node at (8, 4.5) {\tiny{$[784]$}};
    \node at (8.5, 1.96)(hat_x) {\tiny{$g(\bm{h})$}};
    
    %\draw[-latex] (-0.5, -1.6) -- (4.5, -1.6);
    %\draw[-latex] (4.6, -1.6) -- (9, -1.6);
    %\node at (2, -2) {$f$};
    %\node at (6, -2) {$g$};
    
    
    \draw[ultra thick](10, 0) -- (10, 3.92);
    \node at (10, 4.5) {\tiny{$[784]$}};
    \node at (10.25, 1.96)(hat_x) {\tiny{$\bm{n}$}};
    \node at (9.3, 1.96)(a) {\tiny{$+$}};
    \node at (10.8, 1.96)(a) {\tiny{$=$}};
    
    \node at (11.5, 4.5) {\tiny{$[784]$}};
    \draw[ultra thick](11.5, 0) -- (11.5, 3.92);
	 \node at (11.75, 1.96)(hat_x) {\tiny{$\bm{d}$}};

\def\centerx{2}
\def\centery{-1}
	\draw[thick, dashed](3.6, -0.1) -- (3.6, 4.9) -- (9,4.9) -- (9, -0.1) -- (3.65, -0.1);
	\node[circle,draw,outer sep=0pt,inner sep=0.1ex] at (-0.5, 5.25)(a) {1};
	\node[circle,draw,outer sep=0pt,inner sep=0.1ex] at (8.7, 5.25)(a) {2};
	
	\draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4pt},yshift=0pt, thick]
(8,-0.3) -- (11.75,-0.3) node [black,midway,yshift=-0.8cm] {};

		\node[circle,draw,outer sep=0pt,inner sep=0.1ex] at (9.875, -1.2)(a) {3};
			\draw[-latex, thick](12, 1.96)--(12.5, 1.96)--(12.5, -1.8)--(4.6, -1.8);

	 \node at (3, -1.8) {\begin{axis}[width=2.8cm, height=2.8cm,    hide axis,colormap = {whiteblack}{color(0cm)  = (white);color(1cm) = (black)}
]
		
    \addplot3[surf,
    domain=-2:6,
    domain y=-5:3, 
] 
        {exp(-( (x-\centerx)^2 + (y-\centery)^2)/3 )};
    \end{axis}};
	
		\node[circle,draw,outer sep=0pt,inner sep=0.1ex] at (12.85, 0)(a) {4};
	\node at (4, -1.95){\tiny{$\mathcal{P}(\bm{h}|\bm{d})$}};
	
	\draw[-latex, thick](4, -2.2)--(4, -2.8);
	\node at (4, -3) {\tiny{$\mathcal{H}=\{\tilde{\bm{h}}_1, \tilde{\bm{h}}_2, \hdots, \tilde{\bm{h}}_n\}$}};
	\node at (9, -2.1){\tiny{\textsc{Variational Inference}}};
    %\node[left=of x]{\includegraphics[scale=0.3]{images/Reconstruction-Examples/MNIST/mnist_gt.png}};
    %\node[right=of hat_x]{\includegraphics[scale=0.3]{msvlatex_student_files/images/AE/Decoder(Encoder).png}};
  \end{tikzpicture}


==> images/figure3/Mahalanobis_distance_visualization_ssae.tex <==
    \pgfplotsset{
            compat=1.3,
            layers/my layer set/.define layer set={
            background,
            main,
            foreground, 
        }{},
 	        set layers=my layer set,
    }
    
\begin{tikzpicture}[scale=0.8]
    \begin{axis}[ticklabel style = {font=\tiny}, label style={font=\tiny},xlabel=PC-1, ylabel=PC-2,legend style={nodes={scale=0.7, transform shape}},legend style={at={(1.3,0.7)},anchor=west}, scale=0.8]
\addplot[on layer=main,
scatter,
only marks,
point meta=explicit symbolic,
scatter/classes={
0={mark=square,scale=0.4,Red},
1={mark=x,scale=0.4,Blue},
2={mark=+,scale=0.4,Green},
3={mark=pentagon,scale=0.4,Brown},
4={mark=o,scale=0.4,Orange},
5={mark=Mercedes star,scale=0.4,Gray},
6={mark=star,scale=0.4,Purple},
7={mark=diamond,scale=0.4,Cyan},
8={mark=oplus,scale=0.4,VioletRed},
9={mark=triangle,scale=0.4,Black}},
]
table[col sep=comma, meta=label] {images/figure3/data.csv};
\addplot[black, mark=o,
only marks]coordinates {
(-3,-2)}node[pin=150:{\tiny{$\overline{\mathcal{H}}$}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(1.4368732, 0.29129496)
}node[pos=0.8,pin={[pin edge={solid,-}]75:{\tiny{$\delta_{m_0}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(-2.7275455, -2.7784886)
}node[pos=0.1,pin={[pin edge={solid,-}]180:{\tiny{$\delta_{m_1}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(-4.1129346, 5.947219)
}node[pos=0.6,pin={[pin edge={solid,-}]160:{\tiny{$\delta_{m_2}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(5.8840013, 2.9335325)
}node[pos=0.8,pin={[pin edge={solid,-}]85:{\tiny{$\delta_{m_3}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(-1.0261184, -0.68840045)
}node[pos=0.5,pin={[pin edge={solid,-}]90:{\tiny{$\delta_{m_4}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(1.5054904, -1.1637026)
}node[pos=0.7,pin={[pin edge={solid,-}]30:{\tiny{$\delta_{m_5}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(-1.4515756, -1.1309247)
}node[pos=0.9,pin={[pin edge={solid,-}]330:{\tiny{$\delta_{m_6}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(-0.6897279, 1.1449578)
}node[pos=0.6,pin={[pin edge={solid,-}]80:{\tiny{$\delta_{m_7}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(2.0851743, -1.3654587)
}node[pos=0.8,pin={[pin edge={solid,-}]330:{\tiny{$\delta_{m_8}$}}}]{};
\addplot[black,-latex,on layer=foreground,line width=0.7pt]coordinates {
(-3,-2)
(-0.50932276, -3.4935505)
}node[pos=0.5,pin={[pin edge={solid,-}]200:{\tiny{$\delta_{m_9}$}}}]{};
\addlegendentry{$0$}
\addlegendentry{$1$}
\addlegendentry{$2$}
\addlegendentry{$3$}
\addlegendentry{$4$}
\addlegendentry{$5$}
\addlegendentry{$6$}
\addlegendentry{$7$}
\addlegendentry{$8$}
\addlegendentry{$9$}
\end{axis}
\end{tikzpicture}

==> images/figure4/convolution.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[baseline, scale=0.78]
\begin{axis}[scale=0.78,axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.1, xmax=10,
            xmode=log,
            xmajorgrids,
            xminorgrids,
            	title=\Large{(c)},
            xlabel=Convolution level $\gamma$,
            ylabel=$\mathrm{ACC}^h$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.5, transform shape}}]
\addplot[black, mark=o] coordinates {
(0.1, 0.863)
(0.2, 0.859)
(0.3, 0.869)
(0.4, 0.863)
(0.5, 0.861)
(0.6, 0.855)
(0.7, 0.871)
(0.8, 0.867)
(0.9, 0.863)
(1, 0.86)
(1.1, 0.857)
(1.2, 0.85)
(1.3, 0.833)
(1.4, 0.819)
(1.5, 0.814)
(1.6, 0.777)
(1.7, 0.758)
(1.8, 0.736)
(1.9, 0.718)
(2, 0.727)
(3, 0.596)
(4, 0.539)
(5, 0.536)
(6, 0.521)
(7, 0.52)
(8, 0.533)
(9, 0.525)
(10, 0.515)
    };
\addplot[gray, mark=diamond] coordinates {
(0.1, 0.239)
(0.2, 0.239)
(0.3, 0.241)
(0.4, 0.238)
(0.5, 0.242)
(0.6, 0.242)
(0.7, 0.247)
(0.8, 0.247)
(0.9, 0.244)
(1, 0.243)
(1.1, 0.243)
(1.2, 0.238)
(1.3, 0.232)
(1.4, 0.224)
(1.5, 0.216)
(1.6, 0.22)
(1.7, 0.214)
(1.8, 0.208)
(1.9, 0.205)
(2, 0.198)
(3, 0.184)
(4, 0.173)
(5, 0.172)
(6, 0.17)
(7, 0.167)
(8, 0.165)
(9, 0.164)
(10, 0.164)
};
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0.1,0.1)
(10,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.78,axis y line*=right,
            ymin=0, ymax=1.3,
            xmin=0.1, xmax=10,
            axis x line=none,
            xmode=log,
            ylabel=\textcolor{red}{$\delta_r$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.05,0.4)},anchor=west},
            legend style={nodes={scale=0.5, transform shape}}]
\addplot[red, mark=x] coordinates {
(0.1, 0.26710591270020256)
(0.2, 0.26667468625942115)
(0.3, 0.2696304962012446)
(0.4, 0.28699117665052426)
(0.5, 0.3146366476798152)
(0.6, 0.34767632308970997)
(0.7, 0.3776717913146803)
(0.8, 0.4085029239886046)
(0.9, 0.43642100424899827)
(1, 0.46885605141109316)
(1.1, 0.5035361486057753)
(1.2, 0.5370343920316443)
(1.3, 0.5746353363083706)
(1.4, 0.6110984851858429)
(1.5, 0.651694915664365)
(1.6, 0.6839071964557495)
(1.7, 0.7156698000770939)
(1.8, 0.7526756139899446)
(1.9, 0.7794766797451299)
(2, 0.8035521728430022)
(3, 0.9441929209938785)
(4, 0.9909509852090657)
(5, 1.0040873798767995)
(6, 1.011986893862207)
(7, 1.0212981082839823)
(8, 1.0149530340168795)
(9, 1.015880895052075)
(10, 1.0240555922705772)
    };
    \addplot[orange, mark=|] coordinates {
    (0.1, 0.259478213266207)
(0.2, 0.2664152933095628)
(0.3, 0.2637093056465795)
(0.4, 0.2882339846026867)
    (0.5, 0.31641116932335517)
(0.6, 0.36083578109651576)
(0.7, 0.38254207440109855)
(0.8, 0.43355684535508177)
(0.9, 0.4455636563095586)
(1, 0.4952264783786314)
(1.1, 0.5486093609992694)
(1.2, 0.5899777885363489)
(1.3, 0.6366460085246732)
(1.4, 0.6695481008138467)
(1.5, 0.7392972663405356)
(1.6, 0.7588556645241266)
(1.7, 0.7945970949119179)
(1.8, 0.8196581210488504)
(1.9, 0.8538582065668463)
(2, 0.8907115994175565)
(3, 1.0030425972806083)
(4, 1.0384215462668496)
(5, 1.0493566249632225)
(6, 1.047767428407217)
(7, 1.0524468143633627)
(8, 1.0460355090083393)
(9, 1.0560197259499982)
(10, 1.0564028942437063)
    };
\addplot[orange, mark=-] coordinates {
(0.1, 0.26831679893711724)
(0.2, 0.2667172641475818)
(0.3, 0.2705231037532136)
(0.4, 0.2867938826882459)
(0.5, 0.314350168575922)
(0.6, 0.3454446021411874)
(0.7, 0.3769504749907447)
(0.8, 0.40465958887702275)
(0.9, 0.4349696214769278)
(1, 0.4645631912070753)
(1.1, 0.4960151808435003)
(1.2, 0.5276914397072846)
(1.3, 0.5622034248316329)
(1.4, 0.5981810487650019)
(1.5, 0.6316776709152646)
(1.6, 0.6623968896613504)
(1.7, 0.6904713761324667)
(1.8, 0.7286492799362067)
(1.9, 0.7502627653109739)
(2, 0.7708224294388022)
(3, 0.9043015296854241)
(4, 0.9503500044156733)
(5, 0.9648990781601946)
(6, 0.9790907786087331)
(7, 0.9925454565184)
(8, 0.9877194208442497)
(9, 0.9795648099539541)
(10, 0.9935925991502519)
    };
  \end{axis}
\end{tikzpicture}
\begin{tikzpicture}[baseline, scale=0.78]
\begin{axis}[scale=0.78,axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.1, xmax=10,
            	xmode=log,
            xmajorgrids,
            xminorgrids,
            xlabel=Convolution level $\gamma$,
            ylabel=$\mathrm{ACC}^{\delta_m}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.5, transform shape}},]
\addplot[black, mark=o] coordinates {
(0.1, 0.844)
(0.2, 0.836)
(0.3, 0.844)
(0.4, 0.847)
(0.5, 0.837)
(0.6, 0.834)
(0.7, 0.833)
(0.8, 0.822)
(0.9, 0.83)
(1, 0.813)
(1.1, 0.81)
(1.2, 0.791)
(1.3, 0.777)
(1.4, 0.747)
(1.5, 0.755)
(1.6, 0.713)
(1.7, 0.693)
(1.8, 0.675)
(1.9, 0.659)
(2, 0.664)
(3, 0.549)
(4, 0.491)
(5, 0.493)
(6, 0.492)
(7, 0.473)
(8, 0.497)
(9, 0.481)
(10, 0.482)
    };
\addplot[gray, mark=diamond] coordinates {
(0.1, 0.226)
(0.2, 0.226)
(0.3, 0.226)
(0.4, 0.223)
(0.5, 0.232)
(0.6, 0.229)
(0.7, 0.227)
(0.8, 0.228)
(0.9, 0.228)
(1, 0.233)
(1.1, 0.234)
(1.2, 0.23)
(1.3, 0.229)
(1.4, 0.221)
(1.5, 0.219)
(1.6, 0.216)
(1.7, 0.212)
(1.8, 0.205)
(1.9, 0.203)
(2, 0.2)
(3, 0.189)
(4, 0.177)
(5, 0.173)
(6, 0.169)
(7, 0.169)
(8, 0.168)
(9, 0.166)
(10, 0.166)
    };
    \addplot[gray,smooth, mark=none, dashed] coordinates {
(0.1,0.1)
(10,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.78,axis y line*=right,
            ymin=4, ymax=16,
            xmin=0.1, xmax=10,
            xmode=log,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_m$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.01,0.4)},anchor=west},
            legend style={nodes={scale=0.5, transform shape}},]

\addplot[red, mark=x] coordinates {
(0.1, 5.8429204273655)
(0.2, 5.8836218521007355)
(0.3, 5.835267279903696)
(0.4, 5.930187649945964)
(0.5, 6.145132239322621)
(0.6, 6.434529938807662)
(0.7, 6.576325416274937)
(0.8, 6.834243385402113)
(0.9, 7.071938663676547)
(1, 7.326936473749593)
(1.1, 7.623418835540388)
(1.2, 7.923812753136907)
(1.3, 8.273323133552331)
(1.4, 8.657065220318644)
(1.5, 8.982956560968086)
(1.6, 9.312810940396835)
(1.7, 9.645472783476107)
(1.8, 10.015903390541574)
(1.9, 10.345769856060189)
(2, 10.561640454760637)
(3, 12.272865718451872)
(4, 12.77211968858815)
(5, 12.93706738241974)
(6, 13.066429544327763)
(7, 13.142680641348216)
(8, 13.047047141778133)
(9, 13.038126373677112)
(10, 13.142448324539684)
    };
\addplot[orange, mark=|] coordinates {
(0.1, 12.193429823533885)
(0.2, 12.239572087758301)
(0.3, 12.098846625106507)
(0.4, 12.198058872140507)
(0.5, 12.323758928844676)
(0.6, 12.668355424415081)
(0.7, 12.68815978012218)
(0.8, 12.76933777841388)
(0.9, 13.504485521035491)
(1, 13.62630659518774)
(1.1, 13.806100588578774)
(1.2, 13.886419271531793)
(1.3, 13.919572317769545)
(1.4, 13.809832366376508)
(1.5, 14.147121183805226)
(1.6, 14.035961914294463)
(1.7, 13.978248623872817)
(1.8, 13.927748517474056)
(1.9, 14.302253157655578)
(2, 14.49610086484902)
(3, 15.066277685384422)
(4, 15.112271199378473)
(5, 15.355264009450227)
(6, 15.392109267177572)
(7, 15.267790736340498)
(8, 15.337616140484004)
(9, 15.368556612519496)
(10, 15.348711895766183)
    };
\addplot[orange, mark=-] coordinates {
(0.1, 4.669129591106889)
(0.2, 4.636760801086573)
(0.3, 4.677544083397015)
(0.4, 4.797974784543643)
(0.5, 4.941887137301002)
(0.6, 5.193744530401389)
(0.7, 5.351023689069067)
(0.8, 5.549028297864285)
(0.9, 5.7544290663861615)
(1, 5.878003862791496)
(1.1, 6.173160152728915)
(1.2, 6.348357933485161)
(1.3, 6.652842350952023)
(1.4, 6.911884379685927)
(1.5, 7.307168040974578)
(1.6, 7.411626747537623)
(1.7, 7.7260468339785735)
(1.8, 8.13242240350001)
(1.9, 8.298484869953924)
(2, 8.570708680980973)
(3, 9.978095596254095)
(4, 10.34617850937782)
(5, 10.450199857258568)
(6, 10.665117960572267)
(7, 10.774957554538634)
(8, 10.728825398621083)
(9, 10.52358730099687)
(10, 10.771401582018258)
    };
    \end{axis}
\end{tikzpicture}

==> images/figure4/noise_acc_sae.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[baseline, scale=0.78]
\begin{axis}[scale=0.78,
xmode=log,
            log ticks with fixed point,
            axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.01, xmax=10,
            xmajorgrids,
            xminorgrids,
            	title=\Large{(a)},
            xlabel=Noise level $\alpha$,
            ylabel=$\mathrm{ACC}^{h}$,every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},]
\addplot[black, mark=o] coordinates {
(0.01,0.873)
(0.02,0.859)
(0.03,0.864)
(0.04,0.864)
(0.05,0.863)
(0.06,0.869)
(0.07,0.869)
(0.08,0.873)
(0.09,0.871)
(0.1,0.871)
(0.2,0.868)
(0.3,0.855)
(0.4,0.845)
(0.5,0.817)
(0.6,0.793)
(0.7,0.769)
(0.8,0.738)
(0.9,0.703)
(1,0.68)
(2,0.499)
(3,0.421)
(4,0.392)
(5,0.358)
(6,0.349)	
(7,0.326)
(8,0.286)
(9,0.302)
(10, 0.275)
    };
  \label{plot_one_top}

    \addplot[gray, mark=diamond] coordinates {   
(0.010000,0.980000)
(0.020000,0.980000)
(0.030000,0.964000)
(0.040000,0.937000)
(0.050000,0.906000)
(0.060000,0.856000)
(0.070000,0.828000)
(0.080000,0.807000)
(0.090000,0.786000)
(0.100000,0.766000)
(0.200000,0.567000)
(0.300000,0.375000)
(0.400000,0.255000)
(0.500000,0.179000)
(0.600000,0.133000)
(0.700000,0.111000)
(0.800000,0.092000)
(0.900000,0.081000)
(1.000000,0.074000)
(2.000000,0.079000)
(3.000000,0.090000)
(4.000000,0.103000)
(5.000000,0.106000)
(6.000000,0.107000)
(7.000000,0.109000)
(8.000000,0.109000)
(9.000000,0.109000)
(10.000000,0.110000)
};
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0.01,0.1)
(10,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.78,xmode=log,
            log ticks with fixed point,
            axis y line*=right,
            ymin=0, ymax=1.5,
            xmin=0.01, xmax=10,
            axis x line=none,
            ylabel=\textcolor{red}{${\delta}_r$},every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(-0.8,0.5)},anchor=west},
            legend style={nodes={scale=0.9, transform shape}}]
                        \addlegendimage{mark=o}
\addlegendentry{$\mathrm{ACC}_g$}

\addlegendimage{mark=diamond, gray}
\addlegendentry{$\mathrm{ACC}_f$}
\addlegendimage{mark=none, gray, dashed}
\addlegendentry{Random}
\addplot[red, mark=x] coordinates {
(0.01,0.08727)
(0.02,0.12374)
(0.03,0.14935)
(0.04,0.17221)
(0.05,0.1916)
(0.06,0.20772)
(0.07,0.22236)
(0.08,0.23745)
(0.09,0.2486)
(0.1,0.25998)
(0.2,0.35764)
(0.3,0.43056)
(0.4,0.49578)
(0.5,0.55301)	
(0.6,0.60311)
(0.7,0.65036)
(0.8,0.69613)
(0.9,0.73638)
(1,0.7702)
(2,1.01175)
(3,1.13936)
(4,1.2064)
(5,1.258995)
(6,1.29306)
(7,1.31226)
(8,1.33906)	
(9,1.34993)
(10, 1.3636862969374017)
    };

    \addplot[orange, mark=|] coordinates {
(0.01, 0.08312750807795001)
(0.02, 0.12258390671734395)
(0.03, 0.15230219240964676)
(0.04, 0.1791954201983154)
(0.05, 0.20930656253720917)
(0.06, 0.23186168561335266)
(0.07, 0.23957667070783906)
(0.08, 0.26000719569976133)
(0.09, 0.27048951796661536)
(0.1, 0.2885218280993516)
(0.2, 0.42531845486211456)
(0.3, 0.5182981070573495)
(0.4, 0.5737026506983514)
(0.5, 0.6488149945407047)
(0.6, 0.7033399479860463)
(0.7, 0.7521623856642772)
(0.8, 0.7847078027733624)
(0.9, 0.8060964414208853)
(1, 0.8517521277375716)
(2, 1.02754821137981)
(3, 1.1480988912729748)
(4, 1.2025423947827127)
(5, 1.2527494527313991)
(6, 1.2839360227174272)
(7, 1.3023477725567925)
(8, 1.3284738982748039)
(9, 1.3405075496755046)
(10, 1.356294859733464)
    };
\label{std_false_top}
\addplot[orange, mark=-] coordinates {
(0.01, 0.087872182442168)
(0.02, 0.1239365804337927)
(0.03, 0.1488914081497254)
(0.04, 0.1711067455335288)
(0.05, 0.1888000326283356)
(0.06, 0.20408075107891424)
(0.07, 0.219772318452004)
(0.08, 0.2341750218389143)
(0.09, 0.24535910519290544)
(0.1, 0.25575482613386946)
(0.2, 0.34735722722781026)
(0.3, 0.41568919937417803)
(0.4, 0.48148892615832484)
(0.5, 0.5315496833528716)
(0.6, 0.5769504551361601)
(0.7, 0.6209517435930185)
(0.8, 0.6646869743177126)
(0.9, 0.7066369512123996)
(1, 0.7318193325860743)
(2, 0.99588524818257)
(3, 1.1256970643777897)
(4, 1.2123811956639095)
(5, 1.2701991549674116)
(6, 1.310078049960897)
(7, 1.332772177784936)
(8, 1.3654990848510238)
(9, 1.371724091227549)
(10, 1.3831728132023284)
    };
\label{std_true_top}


\addlegendimage{/pgfplots/refstyle=plot_one_top}\addlegendentry{${\delta}_r$}
\addlegendimage{/pgfplots/refstyle=std_true_top}\addlegendentry{${\delta}_{r_{\mathrm{False}}}$}
\addlegendimage{/pgfplots/refstyle=std_false_top}\addlegendentry{${\delta}_{r_{\mathrm{True}}}$}

  \end{axis}
\end{tikzpicture}\\
\begin{tikzpicture}[baseline, scale=0.78]
\begin{axis}[scale=0.78,xmode=log,
            log ticks with fixed point,
            axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.01, xmax=10,
            xmajorgrids,
            xminorgrids,
            xlabel=Noise level $\alpha$,
            ylabel=$\mathrm{ACC}^{\delta_m}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
}]
\addplot[black, mark=o] coordinates {
(0.01, 0.86)
(0.02, 0.843)
(0.03, 0.848)
(0.04, 0.854)
(0.05, 0.856)
(0.06, 0.865)
(0.07, 0.864)
(0.08, 0.862)
(0.09, 0.864)
(0.1, 0.862)
(0.2, 0.858)
(0.3, 0.82)
(0.4, 0.792)
(0.5, 0.753)
(0.6, 0.718)
(0.7, 0.691)
(0.8, 0.642)
(0.9, 0.614)
(1, 0.58)
(2, 0.424)
(3, 0.352)
(4, 0.322)
(5, 0.304)
(6, 0.289)
(7, 0.25)
(8, 0.26)
(9, 0.252)
(10, 0.248)
    };


\label{plot_one_bottom}
\addplot[gray, mark=diamond] coordinates {
(0.010000,0.936000)
(0.020000,0.855000)
(0.030000,0.780000)
(0.040000,0.726000)
(0.050000,0.681000)
(0.060000,0.628000)
(0.070000,0.579000)
(0.080000,0.536000)
(0.090000,0.505000)
(0.100000,0.455000)
(0.200000,0.193000)
(0.300000,0.137000)
(0.400000,0.110000)
(0.500000,0.110000)
(0.600000,0.111000)
(0.700000,0.111000)
(0.800000,0.109000)
(0.900000,0.109000)
(1.000000,0.110000)
(2.000000,0.110000)
(3.000000,0.110000)
(4.000000,0.110000)
(5.000000,0.110000)
(6.000000,0.110000)
(7.000000,0.110000)
(8.000000,0.110000)
(9.000000,0.110000)
(10.000000,0.110000)
    };
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0.01,0.1)
(10,0.1)
    };
\label{Random_bottom}
\end{axis}  
\begin{axis}[scale=0.78,xmode=log,
            log ticks with fixed point,
            axis y line*=right,
            ymin=3, ymax=14,
            xmin=0.01, xmax=10,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_m$},every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(-0.8,0.5)},anchor=west},
            legend style={nodes={scale=0.9, transform shape}}]
                        \addlegendimage{mark=o}
\addlegendentry{$\mathrm{ACC}_g$}

\addlegendimage{mark=diamond, gray}
\addlegendentry{$\mathrm{ACC}_f$}
\addlegendimage{mark=none, gray, dashed}
\addlegendentry{Random}
\addplot[red, mark=x] coordinates {
(0.01, 5.13843227289422)
(0.02, 5.320820114861008)
(0.03, 5.356326515140981)
(0.04, 5.428852160542549)
(0.05, 5.426275500481043)
(0.06, 5.439599361874396)
(0.07, 5.47820054953225)
(0.08, 5.512434300836492)
(0.09, 5.541754635850517)
(0.1, 5.603877971983593)
(0.2, 6.089844562158716)
(0.3, 6.7362646002776305)
(0.4, 7.259281421727414)
(0.5, 7.751918692584218)
(0.6, 8.147375623722022)
(0.7, 8.546365385139183)
(0.8, 8.95815753103678)
(0.9, 9.271474814659381)
(1, 9.534718735531053)
(2, 11.098392030963222)
(3, 11.68659998114136)
(4, 11.903514466306813)
(5, 12.061988360544959)
(6, 12.194142440331637)
(7, 12.253005523489879)
(8, 12.359447044793413)
(9, 12.400683403407282)
(10, 12.44947416569273)
    };
\addplot[orange, mark=|] coordinates {
(0.01, 11.850640473951454)
(0.02, 12.104642325673865)
(0.03, 12.16674499271645)
(0.04, 12.366398858146605)
(0.05, 12.38369122028657)
(0.06, 12.499865528191124)
(0.07, 12.152372540347033)
(0.08, 12.154481108533457)
(0.09, 12.09892442012627)
(0.1, 12.350405457656741)
(0.2, 12.501815281206083)
(0.3, 12.657277689804022)
(0.4, 12.832628358686962)
(0.5, 12.768949735499913)
(0.6, 12.650596956457626)
(0.7, 12.710893394408767)
(0.8, 12.698343540237)
(0.9, 12.641019627774488)
(1, 12.516100614840266)
(2, 12.682395709173784)
(3, 12.820398645000614)
(4, 12.84265931308978)
(5, 12.904110450486819)
(6, 12.955113610229388)
(7, 12.879292300592565)
(8, 12.98770960640464)
(9, 13.007691650775289)
(10, 13.03407446079167)
    };
\label{std_false_bottom}
\addplot[orange, mark=-] coordinates {
(0.01, 4.045747216908158)
(0.02, 4.0574036414356)
(0.03, 4.135591127651038)
(0.04, 4.242807877345603)
(0.05, 4.25586911771002)
(0.06, 4.337708110483924)
(0.07, 4.427636439866959)
(0.08, 4.449090380346723)
(0.09, 4.509607540177481)
(0.1, 4.523807446434992)
(0.2, 5.028655934997031)
(0.3, 5.436530019649886)
(0.4, 5.7955741453542)
(0.5, 6.106225906926614)
(0.6, 6.378700949862077)
(0.7, 6.684080066956402)
(0.8, 6.872508634940707)
(0.9, 7.153161625958353)
(1, 7.375787029824383)
(2, 8.946537977545097)
(3, 9.599379713582278)
(4, 9.92606041003709)
(5, 10.133971996730702)
(6, 10.321995375289074)
(7, 10.374145192181825)
(8, 10.571315138669151)
(9, 10.598928764394305)
(10, 10.676815206360459)
    };
\label{std_true_bottom}
\addlegendimage{/pgfplots/refstyle=plot_one_bottom}\addlegendentry{$\delta_m$}
\addlegendimage{/pgfplots/refstyle=std_false_bottom}\addlegendentry{$\delta_{m_{\mathrm{False}}}$}
\addlegendimage{/pgfplots/refstyle=std_true_bottom}\addlegendentry{$\delta_{m_{\mathrm{True}}}$}

  \end{axis}
\end{tikzpicture}


==> images/figure4/window_mask_acc_sae.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[baseline, scale=0.78]
\begin{axis}[scale=0.78,axis y line*=left,
            ymin=0, ymax=1,
            xmin=1, xmax=14,
            xmajorgrids,
            xminorgrids,
            title=\Large{(b)},
            xlabel=Masking level $\beta$,
            ylabel=$\mathrm{ACC}^{h}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.78, transform shape}}]
\addplot[black, mark=o] coordinates {
(1, 0.871)
(2, 0.867)
(3, 0.87)
(4, 0.857)
(5, 0.862)
(6, 0.854)
(7, 0.806)
(8, 0.733)
(9, 0.587)
(10, 0.394)
(11, 0.321)
(12, 0.21)
(13, 0.166)
(14, 0.126)
    };

\addplot[gray, mark=diamond] coordinates {
(1.000000,0.766000)
(2.000000,0.761000)
(3.000000,0.736000)
(4.000000,0.708000)
(5.000000,0.617000)
(6.000000,0.499000)
(7.000000,0.289000)
(8.000000,0.153000)
(9.000000,0.138000)
(10.000000,0.131000)
(11.000000,0.128000)
(12.000000,0.111000)
(13.000000,0.110000)
(14.000000,0.110000)
};
\addplot[gray,smooth, mark=none, dashed] coordinates {
(1,0.1)
(14,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.78,axis y line*=right,
            ymin=0, ymax=2.2,
            xmin=1, xmax=14,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_r$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.05,0.4)},anchor=west},
            legend style={nodes={scale=0.78, transform shape}}]

\addplot[red, mark=x] coordinates {
(1, 0.2610893484277511)
(2, 0.2613996948080348)
(3, 0.2646145313218816)
(4, 0.2730685581865933)
(5, 0.29306257571145555)
(6, 0.3278986770657249)
(7, 0.38954044823953676)
(8, 0.5037484564210757)
(9, 0.6950811638767723)
(10, 1.030388646760387)
(11, 1.4349993515124824)
(12, 1.7649964245931469)
(13, 1.9972613503703032)
(14, 2.072075877528459)
    };

    \addplot[orange, mark=|] coordinates {
(1, 0.29018467134154385)
(2, 0.29592358829378645)
(3, 0.2884474233625749)
(4, 0.28722087028932725)
(5, 0.3010051088372677)
(6, 0.35841567807537006)
(7, 0.4036106060784774)
(8, 0.5005323376579797)
(9, 0.7218042244456162)
(10, 1.0489539852520668)
(11, 1.4458587311834505)
(12, 1.769889377604653)
(13, 1.9969107530416443)
(14, 2.071593832039184)
    };
\addplot[orange, mark=-] coordinates {
(1, 0.25678016742214926)
(2, 0.25610364194343854)
(3, 0.2610532945801688)
(4, 0.27070708720562364)
(5, 0.2917910332852815)
(6, 0.322681484855645)
(7, 0.38615383456614416)
(8, 0.504919948521685)
(9, 0.6762794193879604)
(10, 1.0018338367960264)
(11, 1.4120288879717116)
(12, 1.746589601359386)
(13, 1.9990227851419995)
(14, 2.0754195898905716)
    };
  \end{axis}
\end{tikzpicture}\\
\begin{tikzpicture}[baseline, scale=0.78]
\begin{axis}[scale=0.78,axis y line*=left,
            ymin=0, ymax=1,
            xmin=1, xmax=14,
            xmajorgrids,
            xminorgrids,
            xlabel=Masking level $\beta$,
            ylabel=$\mathrm{ACC}^{\delta_m}$,
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={nodes={scale=0.78, transform shape}},]

            
            
\addplot[black, mark=o] coordinates {
(1, 0.866)
(2, 0.861)
(3, 0.862)
(4, 0.851)
(5, 0.841)
(6, 0.829)
(7, 0.778)
(8, 0.659)
(9, 0.482)
(10, 0.299)
(11, 0.193)
(12, 0.16)
(13, 0.142)
(14, 0.115)
    };
\addplot[gray, mark=diamond] coordinates {
(1.000000,0.762000)
(2.000000,0.756000)
(3.000000,0.730000)
(4.000000,0.700000)
(5.000000,0.608000)
(6.000000,0.487000)
(7.000000,0.275000)
(8.000000,0.150000)
(9.000000,0.135000)
(10.000000,0.111000)
(11.000000,0.110000)
(12.000000,0.110000)
(13.000000,0.110000)
(14.000000,0.110000)
    };
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0,0.1)
(14,0.1)
    };
\end{axis}  
\begin{axis}[scale=0.78,axis y line*=right,
            ymin=3, ymax=17.5,
            xmin=1, xmax=14,
            axis x line=none,
            ylabel=\textcolor{red}{$\delta_m$},
            every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    anchor=south,
},
            legend style={at={(0.01,0.4)},anchor=west},
            legend style={nodes={scale=0.78, transform shape}},]
\addplot[red, mark=x] coordinates {
(1, 5.5846937824643526)
(2, 5.649589056348564)
(3, 5.6160404930997165)
(4, 5.729722398821481)
(5, 5.87001664678334)
(6, 6.300607839274489)
(7, 7.161627904927534)
(8, 8.73866704344245)
(9, 11.170564281530737)
(10, 14.408680743386073)
(11, 16.16476758260979)
(12, 16.31917491177355)
(13, 15.819140792413632)
(14, 15.399848278998837)
    };

\addplot[orange, mark=|] coordinates {
(1, 12.239018713872184)
(2, 12.39472170835417)
(3, 12.083315443410266)
(4, 11.906713923364743)
(5, 12.072713850419913)
(6, 12.497570977966847)
(7, 13.117857458514939)
(8, 13.715356792226135)
(9, 14.709092859062412)
(10, 16.286807391956764)
(11, 17.059778319289272)
(12, 16.850337237224778)
(13, 16.24803318647567)
(14, 15.744300623379031)
    };

\addplot[orange, mark=-] coordinates {
(1, 4.555040733031732)
(2, 4.560653587557879)
(3, 4.58067628991775)
(4, 4.648204493819194)
(5, 4.697330730756925)
(6, 5.022344031413943)
(7, 5.462035410202079)
(8, 6.163475534587764)
(9, 7.3677472625236655)
(10, 10.005447363292243)
(11, 12.422416989343763)
(12, 13.53057270315461)
(13, 13.22766421420781)
(14, 12.749062846159953)
    };
\end{axis}

\end{tikzpicture}

==> images/figure5/ACC_AUC.tex <==
%     \begin{tabular}{llll}
%     \toprule
%     \multicolumn{1}{c}{\bf $\alpha$}&\multicolumn{1}{c}{\bf METHOD; INPUT}  &\multicolumn{1}{c}{\bf ACC}&\multicolumn{1}{c}{\bf AUC}
%     \\ \midrule
%     \multirow{5}*{$0.1$} & Our Method; $\bm{d}$ & 0.862 &0.904\\
%      & MC Dropout; $\bm{d}$       & 0.915& 0.745
% \\
%     & MC Dropout; $g(\overline{\mathcal{H}})$       &0.886 &0.754
% \\
%      & EDL; $\bm{d}$         & 0.666    &0.746%\\
%      %& EDL; $g(\overline{\mathcal{H}})$         & 0.918 &0.941
% \\ \midrule
%     \multirow{5}*{$0.5$} & Our Method; $\bm{d}$ & 0.753 &0.881
% \\
%     & MC Dropout; $\bm{d}$       & 0.755   &0.555%\\
%     %& MC Dropout; $g(\overline{\mathcal{H}})$       & 0.792    &0.654
% \\          
%     & EDL; $\bm{d}$         & 0.125 &0.717%\\
%     %& EDL; $g(\overline{\mathcal{H}})$         & 0.856  &0.900
% \\\midrule
%      \multirow{5}*{$1.0$} & Our Method; $\bm{d}$  & 0.580 &0.828
% \\
%       & MC Dropout; $\bm{d}$       &0.570   & 0.472%\\
%   %& MC Dropout; $g(\overline{\mathcal{H}})$       & 0.675  &0.597
% \\
%     & EDL; $\bm{d}$         & 0.089 &0.885%\\
% %       & EDL; $g(\overline{\mathcal{H}})$         & 0.751   &0.837
% \\
%       \bottomrule
%     \end{tabular}}



\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[scale=0.8]
\begin{axis}[scale=0.8,
			axis y line*=left,
            ymin=0, ymax=1,
            xmin=0.1, xmax=1,
            xmajorgrids,
            xtick={0.1, 0.5,1.0},
            %xminorgrids,
            xlabel=Noise Level $\alpha$,
            ylabel=ACC / AUC,
            	title=Performance Evaluation, 
            width=6.5cm, height=5.5cm,
            legend style={at={(1.1,0.5)},anchor=west}, 
            legend style={nodes={scale=0.5, transform shape}}
            ]
\addplot[black,  mark=o,forget plot] coordinates { %ACC
(0.1, 0.862)
(0.5, 0.753)
(1.0, 0.580)
    };
    \addplot[black,  mark=o, dashed,forget plot] coordinates { %AUC
(0.1, 0.904)
(0.5, 0.881)
(1.0, 0.828)
    };
% MC Dropout
\addplot[cyan, mark=x,forget plot] coordinates { %ACC
(0.1, 0.915)
(0.5, 0.755)
(1.0, 0.570) 
    };
% MC Dropout
\addplot[cyan, mark=x, dashed,forget plot] coordinates { %AUC
(0.1, 0.745)
(0.5,0.555)
(1.0, 0.472) 
    };
% Evidential Deep Learning

\addplot[orange, mark=|,,forget plot] coordinates { %ACC
(0.1, 0.666 )
(0.5,0.125)
(1.0, 0.089)
    };
    
\addplot[orange, mark=|, dashed,forget plot] coordinates { %AUC
(0.1, 0.746)
(0.5,0.717)
(1.0, 0.885)
    };
    
\addplot[gray,smooth, mark=none] coordinates {
(0,0.1)
(1,0.1)
    };
\addlegendentry{Accuracy (ACC)}
 
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0,0.5)
(1,0.5)
    };
\addlegendentry{Area Under the Curve (AUC)}

\end{axis}
\end{tikzpicture}

==> images/figure5/ROC.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[scale=0.8]
\begin{axis}[scale=0.8,
			axis y line*=left,
            ymin=0, ymax=1,
            xmin=0, xmax=1,
            xmajorgrids,
            xminorgrids,
            xlabel=False Positive Rate,
            ylabel=True Positive Rate,
            	title=U-ROC-Curve $\alpha \equal 0.1$, 
            width=6.5cm, height=5.5cm,
            legend style={at={(1.4,0.5)},anchor=west}, 
            legend style={nodes={scale=0.7, transform shape}}, legend cell align={left}]
\addplot[black, mark=o] coordinates {
(0.0,0.0)
(0.0,0.002320185614849188)
(0.0,0.002320185614849188)
(0.0,0.0069605568445475635)
(0.0,0.019721577726218097)
(0.0,0.04524361948955916)
(0.0,0.08352668213457076)
(0.0,0.12296983758700696)
(0.0,0.1716937354988399)
(0.0,0.22621809744779584)
(0.0,0.28306264501160094)
(0.0,0.351508120649652)
(0.0,0.40835266821345706)
(0.0,0.4779582366589327)
(0.007246376811594203,0.5382830626450116)
(0.021739130434782608,0.5823665893271461)
(0.036231884057971016,0.62877030162413)
(0.043478260869565216,0.6647331786542924)
(0.050724637681159424,0.7018561484918794)
(0.050724637681159424,0.7354988399071926)
(0.07971014492753623,0.7645011600928074)
(0.10144927536231885,0.7865429234338747)
(0.12318840579710146,0.8051044083526682)
(0.14492753623188406,0.8225058004640371)
(0.16666666666666666,0.8387470997679815)
(0.1956521739130435,0.851508120649652)
(0.30434782608695654,0.8747099767981439)
(0.34782608695652173,0.8874709976798144)
(0.41304347826086957,0.9002320185614849)
(0.43478260869565216,0.9095127610208816)
(0.463768115942029,0.9245939675174014)
(0.5,0.9385150812064965)
(0.5289855072463768,0.9477958236658933)
(0.5869565217391305,0.9535962877030162)
(0.6231884057971014,0.9582366589327146)
(0.6594202898550725,0.9605568445475638)
(0.6884057971014492,0.9651972157772621)
(0.7318840579710145,0.9709976798143851)
(0.7463768115942029,0.974477958236659)
(0.7536231884057971,0.9756380510440835)
(0.7753623188405797,0.9802784222737819)
(0.782608695652174,0.9837587006960556)
(0.8043478260869565,0.9849187935034803)
(0.8188405797101449,0.9849187935034803)
(0.8260869565217391,0.9895591647331786)
(0.8333333333333334,0.9895591647331786)
(0.855072463768116,0.9895591647331786)
(0.855072463768116,0.9907192575406032)
(0.855072463768116,0.9930394431554525)
(0.8913043478260869,0.994199535962877)
(0.8985507246376812,0.994199535962877)
(0.9130434782608695,0.9953596287703016)
(0.927536231884058,0.9965197215777262)
(1.0,1.0)
    };
    %\addlegendentry{Our method, Input = $\bm{d}$};

\addplot[cyan, mark=x] coordinates {
(0.0,0.0)
(0.0,0.0011587485515643105)
(0.0,0.0011574074074074073)
(0.0,0.002325581395348837)
(0.0,0.0)
(0.0,0.0011614401858304297)
(0.0,0.0)
(0.0,0.005813953488372093)
(0.0,0.003464203233256351)
(0.0,0.0069605568445475635)
(0.0,0.0069605568445475635)
(0.0,0.017341040462427744)
(0.0,0.011614401858304297)
(0.0,0.016203703703703703)
(0.0,0.01853997682502897)
(0.0,0.031286210892236384)
(0.0,0.025433526011560695)
(0.007042253521126761,0.03496503496503497)
(0.007352941176470588,0.04050925925925926)
(0.0,0.03841676367869616)
(0.0,0.0429732868757259)
(0.0,0.04519119351100811)
(0.0,0.06936416184971098)
(0.0,0.06511627906976744)
(0.007407407407407408,0.09364161849710982)
(0.007518796992481203,0.0922722029988466)
(0.0,0.10788863109048724)
(0.0072992700729927005,0.11471610660486674)
(0.014598540145985401,0.13557358053302435)
(0.0,0.13921113689095127)
(0.014814814814814815,0.1699421965317919)
(0.030303030303030304,0.16589861751152074)
(0.0,0.19674039580908032)
(0.037037037037037035,0.20346820809248556)
(0.014285714285714285,0.24302325581395348)
(0.021739130434782608,0.23781902552204176)
(0.022058823529411766,0.2534722222222222)
(0.05,0.28255813953488373)
(0.051094890510948905,0.30243337195828507)
(0.04964539007092199,0.3410942956926659)
(0.07246376811594203,0.37935034802784223)
(0.04895104895104895,0.40606767794632437)
(0.11188811188811189,0.4200700116686114)
(0.08695652173913043,0.46867749419953597)
(0.10218978102189781,0.5052143684820394)
(0.13286713286713286,0.5262543757292882)
(0.20588235294117646,0.6018518518518519)
(0.2302158273381295,0.6445993031358885)
(0.28888888888888886,0.6763005780346821)
(0.4460431654676259,0.7630662020905923)
(0.5912408759124088,0.8424101969872537)
(1.0,1.0)
    };
%\addlegendentry{MC Dropout, Input = $\bm{d}$};

% \addplot[blue, mark=star] coordinates {
% (0.0,0.0)
% (0.0,0.0011641443538998836)
% (0.0,0.002325581395348837)
% (0.0,0.0034802784222737818)
% (0.0,0.00580046403712297)
% (0.0,0.008111239860950173)
% (0.0,0.013888888888888888)
% (0.0,0.01627906976744186)
% (0.0,0.010526315789473684)
% (0.0,0.013937282229965157)
% (0.0,0.016260162601626018)
% (0.0072992700729927005,0.03244495944380069)
% (0.0,0.03236994219653179)
% (0.007194244604316547,0.026713124274099883)
% (0.0,0.04428904428904429)
% (0.0,0.04524361948955916)
% (0.0,0.04387990762124711)
% (0.0,0.06511627906976744)
% (0.007194244604316547,0.06736353077816493)
% (0.0,0.0777262180974478)
% (0.0,0.07566938300349244)
% (0.0,0.09941520467836257)
% (0.0,0.09930715935334873)
% (0.0,0.11020881670533643)
% (0.0,0.12384259259259259)
% (0.007352941176470588,0.15625)
% (0.0,0.15144508670520232)
% (0.0072992700729927005,0.1633835457705678)
% (0.014184397163120567,0.1990686845168801)
% (0.014184397163120567,0.20721769499417927)
% (0.021897810218978103,0.2190034762456547)
% (0.021897810218978103,0.23406720741599074)
% (0.03571428571428571,0.25813953488372093)
% (0.0364963503649635,0.27578215527230593)
% (0.050359712230215826,0.32171893147502906)
% (0.06569343065693431,0.3267670915411356)
% (0.06521739130434782,0.37819025522041766)
% (0.08029197080291971,0.388180764774044)
% (0.08695652173913043,0.43503480278422274)
% (0.07913669064748201,0.4727061556329849)
% (0.15384615384615385,0.49941656942823803)
% (0.1956521739130435,0.5638051044083526)
% (0.1897810218978102,0.6141367323290846)
% (0.22857142857142856,0.6674418604651163)
% (0.36428571428571427,0.7034883720930233)
% (0.38235294117647056,0.7708333333333334)
% (0.5671641791044776,0.848729792147806)
% (1.0,1.0)
% };
%\addlegendentey{Dropout Classifier $g(\overline{\mathcal{H}})$};
% Evidential Deep Learning

\addplot[orange, mark=|] coordinates {
(0.0,0.0)
(0.0,0.006006006006006006)
(0.0,0.021021021021021023)
(0.0,0.06456456456456457)
(0.0,0.11861861861861862)
(0.0,0.16366366366366367)
(0.0,0.21021021021021022)
(0.0029940119760479044,0.25375375375375375)
(0.008982035928143712,0.2927927927927928)
(0.011976047904191617,0.32732732732732733)
(0.017964071856287425,0.35435435435435436)
(0.03592814371257485,0.3963963963963964)
(0.038922155688622756,0.42492492492492495)
(0.059880239520958084,0.44894894894894893)
(0.059880239520958084,0.466966966966967)
(0.08383233532934131,0.487987987987988)
(0.09580838323353294,0.4984984984984985)
(0.10778443113772455,0.5075075075075075)
(0.10778443113772455,0.5180180180180181)
(0.12574850299401197,0.5315315315315315)
(0.1407185628742515,0.5480480480480481)
(0.1467065868263473,0.5570570570570571)
(0.15568862275449102,0.5645645645645646)
(0.16766467065868262,0.5675675675675675)
(0.17365269461077845,0.5735735735735735)
(0.18562874251497005,0.5825825825825826)
(0.18562874251497005,0.5900900900900901)
(0.20658682634730538,0.5960960960960962)
(0.2155688622754491,0.6051051051051051)
(0.218562874251497,0.6141141141141141)
(0.24251497005988024,0.6276276276276276)
(0.25149700598802394,0.6351351351351351)
(0.26047904191616766,0.6411411411411412)
(0.2694610778443114,0.6471471471471472)
(0.281437125748503,0.6561561561561562)
(0.2964071856287425,0.6681681681681682)
(0.30538922155688625,0.6726726726726727)
(0.3083832335329341,0.6771771771771772)
(0.32335329341317365,0.6786786786786787)
(0.3323353293413174,0.6876876876876877)
(0.33532934131736525,0.6936936936936937)
(0.3383233532934132,0.6951951951951952)
(0.344311377245509,0.6996996996996997)
(0.3502994011976048,0.7042042042042042)
(0.36227544910179643,0.7102102102102102)
(0.38023952095808383,0.7177177177177178)
(0.38622754491017963,0.7222222222222222)
(0.38622754491017963,0.7267267267267268)
(0.39520958083832336,0.7267267267267268)
(0.4041916167664671,0.7267267267267268)
(0.4101796407185629,0.7312312312312312)
(0.4101796407185629,0.7327327327327328)
(0.4161676646706587,0.7357357357357357)
(0.4251497005988024,0.7387387387387387)
(0.4341317365269461,0.7447447447447447)
(0.4491017964071856,0.7492492492492493)
(0.45209580838323354,0.7537537537537538)
(0.45209580838323354,0.7567567567567568)
(0.46107784431137727,0.7582582582582582)
(0.46107784431137727,0.7597597597597597)
(0.47305389221556887,0.7612612612612613)
(0.4820359281437126,0.7657657657657657)
(0.4820359281437126,0.7672672672672672)
(0.48502994011976047,0.7702702702702703)
(0.48502994011976047,0.7747747747747747)
(0.5,0.7792792792792793)
(0.5089820359281437,0.7792792792792793)
(0.5299401197604791,0.7822822822822822)
(0.5299401197604791,0.7852852852852853)
(0.5359281437125748,0.7897897897897898)
(0.5359281437125748,0.7912912912912913)
(0.5389221556886228,0.7942942942942943)
(0.5419161676646707,0.7957957957957958)
(0.5508982035928144,0.7972972972972973)
(0.5538922155688623,0.7987987987987988)
(0.562874251497006,0.8018018018018018)
(0.5688622754491018,0.8048048048048048)
(0.5688622754491018,0.8063063063063063)
(0.5778443113772455,0.8078078078078078)
(0.5808383233532934,0.8093093093093093)
(0.592814371257485,0.8108108108108109)
(0.5988023952095808,0.8123123123123123)
(0.6017964071856288,0.8138138138138138)
(0.6047904191616766,0.8153153153153153)
(0.6137724550898204,0.8168168168168168)
(0.6197604790419161,0.8183183183183184)
(0.7604790419161677,0.8843843843843844)
(0.7634730538922155,0.8858858858858859)
(1.0, 1.0)
    };
   % \addlegendentry{EDL, Input = $\bm{d}$};    
% \addplot[red, mark=10-pointed star] coordinates {
% (0.0,0.0)
% (0.0,0.0032679738562091504)
% (0.0,0.020697167755991286)
% (0.0,0.1111111111111111)
% (0.0,0.23093681917211328)
% (0.0,0.3464052287581699)
% (0.0,0.4411764705882353)
% (0.0,0.5152505446623094)
% (0.0,0.5686274509803921)
% (0.0,0.6241830065359477)
% (0.012195121951219513,0.6677559912854031)
% (0.024390243902439025,0.7058823529411765)
% (0.024390243902439025,0.7374727668845316)
% (0.024390243902439025,0.7549019607843137)
% (0.06097560975609756,0.7701525054466231)
% (0.06097560975609756,0.7821350762527233)
% (0.07317073170731707,0.7941176470588235)
% (0.08536585365853659,0.8137254901960784)
% (0.12195121951219512,0.8235294117647058)
% (0.12195121951219512,0.8387799564270153)
% (0.12195121951219512,0.8529411764705882)
% (0.12195121951219512,0.8627450980392157)
% (0.13414634146341464,0.8703703703703703)
% (0.13414634146341464,0.8714596949891068)
% (0.14634146341463414,0.8747276688453159)
% (0.15853658536585366,0.8790849673202614)
% (0.15853658536585366,0.8845315904139434)
% (0.17073170731707318,0.8867102396514162)
% (0.18292682926829268,0.8888888888888888)
% (0.18292682926829268,0.8954248366013072)
% (0.18292682926829268,0.900871459694989)
% (0.18292682926829268,0.9019607843137255)
% (0.18292682926829268,0.9030501089324618)
% (0.18292682926829268,0.906318082788671)
% (0.18292682926829268,0.9106753812636166)
% (0.18292682926829268,0.9150326797385621)
% (0.18292682926829268,0.9172113289760349)
% (0.18292682926829268,0.9193899782135077)
% (0.18292682926829268,0.9215686274509803)
% (0.18292682926829268,0.9215686274509803)
% (0.18292682926829268,0.9237472766884531)
% (0.18292682926829268,0.9237472766884531)
% (0.2073170731707317,0.9259259259259259)
% (0.2073170731707317,0.9259259259259259)
% (0.2073170731707317,0.9270152505446623)
% (0.21951219512195122,0.9291938997821351)
% (0.23170731707317074,0.9302832244008714)
% (0.23170731707317074,0.9313725490196079)
% (0.23170731707317074,0.9324618736383442)
% (0.23170731707317074,0.9324618736383442)
% (0.23170731707317074,0.9324618736383442)
% (0.24390243902439024,0.9324618736383442)
% (0.24390243902439024,0.934640522875817)
% (0.524390243902439,0.971677559912854)
% (0.524390243902439,0.9760348583877996)
% (0.524390243902439,0.9760348583877996)
% (0.524390243902439,0.9760348583877996)  
% (1.0,1.0)
% };
    %\addlegendentry{Evidential Deep Learning  $g(\overline{\mathcal{H}})$}; 
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0,0)
(1,1)
    };
%\addlegendentry{Random}
\end{axis}
\end{tikzpicture}

==> images/figure5/ROC1.tex <==
\pgfplotsset{compat=1.3,small}
\begin{tikzpicture}[scale=0.8]
\begin{axis}[scale=0.8,
			axis y line*=left,
            ymin=0, ymax=1,
            xmin=0, xmax=1,
            xmajorgrids,
            xminorgrids,
            xlabel=False Positive Rate,
            ylabel=True Positive Rate,
            	title=U-ROC-Curve $\alpha \equal 0.5$, 
            width=6.5cm, height=5.5cm,
           ]
\addplot[black, mark=o] coordinates {
(0.0,0.0)
(0.0,0.0013315579227696406)
(0.0,0.0013315579227696406)
(0.0,0.002663115845539281)
(0.0,0.010652463382157125)
(0.0,0.022636484687083888)
(0.0,0.0426098535286285)
(0.0,0.06790945406125166)
(0.0,0.085219707057257)
(0.0,0.10918774966711052)
(0.0,0.14513981358189082)
(0.0,0.1810918774966711)
(0.0,0.21438082556591212)
(0.0,0.27030625832223704)
(0.0,0.30492676431424764)
(0.004016064257028112,0.35286284953395475)
(0.012048192771084338,0.39280958721704395)
(0.01606425702811245,0.45006657789613846)
(0.01606425702811245,0.4966711051930759)
(0.020080321285140562,0.5352862849533955)
(0.024096385542168676,0.5778961384820239)
(0.04417670682730924,0.625832223701731)
(0.04819277108433735,0.6524633821571239)
(0.0642570281124498,0.681757656458056)
(0.10843373493975904,0.7070572569906791)
(0.1285140562248996,0.7350199733688415)
(0.1606425702811245,0.7509986684420772)
(0.18072289156626506,0.7723035952063915)
(0.21686746987951808,0.7909454061251664)
(0.23694779116465864,0.8095872170439414)
(0.2570281124497992,0.8202396804260985)
(0.30120481927710846,0.8308921438082557)
(0.3253012048192771,0.8402130492676432)
(0.3493975903614458,0.8588548601864181)
(0.37751004016064255,0.8681757656458056)
(0.40160642570281124,0.8841544607190412)
(0.40562248995983935,0.8961384820239681)
(0.42570281124497994,0.9174434087882823)
(0.4497991967871486,0.9254327563249002)
(0.46987951807228917,0.929427430093209)
(0.4979919678714859,0.9374167776298269)
(0.5381526104417671,0.9400798934753661)
(0.5582329317269076,0.948069241011984)
(0.5863453815261044,0.9507323568575233)
(0.6144578313253012,0.9600532623169108)
(0.6305220883534136,0.9680426098535286)
(0.678714859437751,0.9707057256990679)
(0.7068273092369478,0.9720372836218375)
(0.7469879518072289,0.9773635153129161)
(0.7710843373493976,0.9800266311584553)
 (1.0,1.0)
    };
  %  \addlegendentry{Our method, Input = $\bm{d}$};

\addplot[cyan, mark=x] coordinates {
(0.0,0.0)
(0.0,0.0013054830287206266)
(0.0,0.00392156862745098)
(0.0,0.00130718954248366)
(0.0,0.003931847968545216)
(0.0,0.011795543905635648)
(0.0,0.00904392764857881)
(0.0,0.0078125)
(0.0,0.005201560468140442)
(0.0,0.016861219195849545)
(0.0,0.01568627450980392)
(0.0,0.02490170380078637)
(0.0,0.02860858257477243)
(0.004201680672268907,0.028871391076115485)
(0.0,0.025974025974025976)
(0.008658008658008658,0.04681404421326398)
(0.004201680672268907,0.03674540682414698)
(0.004310344827586207,0.036458333333333336)
(0.004201680672268907,0.05249343832020997)
(0.004273504273504274,0.06005221932114883)
(0.008733624454148471,0.0609597924773022)
(0.02092050209205021,0.06176084099868594)
(0.017316017316017316,0.0858257477243173)
(0.022321428571428572,0.09149484536082474)
(0.0205761316872428,0.09379128137384413)
(0.030434782608695653,0.10649350649350649)
(0.02643171806167401,0.11513583441138421)
(0.02575107296137339,0.1303780964797914)
(0.056768558951965066,0.14785992217898833)
(0.05333333333333334,0.1393548387096774)
(0.06896551724137931,0.18359375)
(0.07627118644067797,0.20287958115183247)
(0.13675213675213677,0.21148825065274152)
(0.14285714285714285,0.2690288713910761)
(0.15677966101694915,0.2696335078534031)
(0.19913419913419914,0.31209362808842656)
(0.2782608695652174,0.36753246753246754)
(0.35294117647058826,0.452755905511811)
(0.502262443438914,0.5430038510911425)
(1.0,1.0)
    };
%\addlegendentry{MC Dropout, Input = $\bm{d}$};

% \addplot[blue, mark=star] coordinates {
% (0.0,0.0)
% (0.0,0.0013227513227513227)
% (0.0,0.0026455026455026454)
% (0.004132231404958678,0.002638522427440633)
% (0.0,0.006570302233902759)
% (0.004149377593360996,0.00922266139657444)
% (0.0041841004184100415,0.00788436268068331)
% (0.004149377593360996,0.011857707509881422)
% (0.0,0.022397891963109356)
% (0.0,0.01844532279314888)
% (0.0,0.021052631578947368)
% (0.0,0.015748031496062992)
% (0.0,0.03571428571428571)
% (0.0,0.030104712041884817)
% (0.00816326530612245,0.033112582781456956)
% (0.0125,0.046052631578947366)
% (0.012345679012345678,0.04227212681638045)
% (0.01282051282051282,0.057441253263707574)
% (0.012711864406779662,0.056282722513089)
% (0.012711864406779662,0.07460732984293193)
% (0.016666666666666666,0.06842105263157895)
% (0.01646090534979424,0.07793923381770146)
% (0.024793388429752067,0.08311345646437995)
% (0.02092050209205021,0.07752956636005257)
% (0.01694915254237288,0.10078534031413612)
% (0.03278688524590164,0.12698412698412698)
% (0.03829787234042553,0.1450980392156863)
% (0.03361344537815126,0.14566929133858267)
% (0.041666666666666664,0.15657894736842104)
% (0.012244897959183673,0.17483443708609273)
% (0.0423728813559322,0.193717277486911)
% (0.05,0.22105263157894736)
% (0.04132231404958678,0.20316622691292877)
% (0.06147540983606557,0.23015873015873015)
% (0.07142857142857142,0.2585301837270341)
% (0.08536585365853659,0.2838196286472148)
% (0.08786610878661087,0.30223390275952694)
% (0.1111111111111111,0.3289299867899604)
% (0.12658227848101267,0.36041939711664484)
% (0.13559322033898305,0.4083769633507853)
% (0.15879828326180256,0.42633637548891784)
% (0.20081967213114754,0.4576719576719577)
% (0.225,0.5039473684210526)
% (0.301255230125523,0.5479632063074902)
% (0.4083333333333333,0.6039473684210527)
% (0.5443037974683544,0.6920052424639581)
% (0.6122448979591837,0.7721854304635761)
% (1.0,1.0)
% };
%\addlegendentry{Dropout Classifier $g(\overline{\mathcal{H}})$};
% Evidential Deep Learning

\addplot[orange, mark=|] coordinates {
(0.0,0.008)
(0.0,0.048)
(0.002285714285714286,0.152)
(0.012571428571428572,0.32)
(0.038857142857142854,0.44)
(0.05714285714285714,0.544)
(0.09828571428571428,0.584)
(0.16228571428571428,0.608)
(0.21942857142857142,0.64)
(0.28114285714285714,0.664)
(0.3302857142857143,0.68)
(0.37942857142857145,0.688)
(0.4308571428571429,0.696)
(0.46514285714285714,0.704)
(0.528,0.704)
(0.5542857142857143,0.728)
(0.5725714285714286,0.736)
(0.6114285714285714,0.752)
(0.6422857142857142,0.76)
(0.6525714285714286,0.768)
(0.6628571428571428,0.776)
(0.7314285714285714,0.784)
(0.784,0.792)
(0.7874285714285715,0.8)
(0.7965714285714286,0.808)
(0.8228571428571428,0.816)
(0.8285714285714286,0.832)
(0.8422857142857143,0.84)
(0.8445714285714285,0.848)
(0.8571428571428571,0.856)
(0.864,0.864)
(0.8662857142857143,0.872)
(0.8708571428571429,0.88)
(0.9074285714285715,0.888)
(0.9302857142857143,0.928)
(1.0, 1.0)
    };
%    \addlegendentry{EDL, Input = $\bm{d}$};    
% \addplot[red, mark=asterisk] coordinates {
% (0.0,0.0)
% (0.0,0.002336448598130841)
% (0.0,0.018691588785046728)
% (0.0,0.06191588785046729)
% (0.0,0.14369158878504673)
% (0.0,0.23130841121495327)
% (0.0,0.29906542056074764)
% (0.0,0.35630841121495327)
% (0.0,0.411214953271028)
% (0.0,0.46845794392523366)
% (0.0,0.5128504672897196)
% (0.013888888888888888,0.5467289719626168)
% (0.020833333333333332,0.5794392523364486)
% (0.034722222222222224,0.6121495327102804)
% (0.04861111111111111,0.639018691588785)
% (0.05555555555555555,0.655373831775701)
% (0.0625,0.6799065420560748)
% (0.06944444444444445,0.6915887850467289)
% (0.0763888888888889,0.7044392523364486)
% (0.0763888888888889,0.7242990654205608)
% (0.0763888888888889,0.7313084112149533)
% (0.08333333333333333,0.7453271028037384)
% (0.1111111111111111,0.7535046728971962)
% (0.125,0.7651869158878505)
% (0.13194444444444445,0.772196261682243)
% (0.1527777777777778,0.7815420560747663)
% (0.1597222222222222,0.7862149532710281)
% (0.16666666666666666,0.7967289719626168)
% (0.16666666666666666,0.8037383177570093)
% (0.16666666666666666,0.8107476635514018)
% (0.16666666666666666,0.8189252336448598)
% (0.16666666666666666,0.8247663551401869)
% (0.16666666666666666,0.8271028037383178)
% (0.18055555555555555,0.8317757009345794)
% (0.1875,0.8329439252336449)
% (0.2013888888888889,0.8399532710280374)
% (0.20833333333333334,0.8411214953271028)
% (0.20833333333333334,0.8422897196261683)
% (0.2152777777777778,0.8469626168224299)
% (0.2152777777777778,0.8504672897196262)
% (0.2152777777777778,0.8516355140186916)
% (0.2152777777777778,0.8563084112149533)
% (0.2152777777777778,0.8574766355140186)
% (0.2152777777777778,0.8586448598130841)
% (0.2152777777777778,0.8633177570093458)
% (0.2152777777777778,0.8644859813084113)
% (0.2222222222222222,0.866822429906542)
% (0.2222222222222222,0.8679906542056075)
% (0.22916666666666666,0.8726635514018691)
% (0.24305555555555555,0.8773364485981309)
% (0.24305555555555555,0.8796728971962616)
% (0.2569444444444444,0.8820093457943925)
% (0.2569444444444444,0.8820093457943925)
% (0.5138888888888888,0.9439252336448598)
% (0.5208333333333334,0.9462616822429907)
% (0.5208333333333334,0.9462616822429907)
% (0.5208333333333334,0.9462616822429907) 
% (1.0,1.0)
% };
    %\addlegendentry{Evidential Deep Learning  $g(\overline{\mathcal{H}})$}; 
\addplot[gray,smooth, mark=none, dashed] coordinates {
(0,0)
(1,1)
    };
%\addlegendentry{Random};
\end{axis}
\end{tikzpicture}


==> images/figure5/ROC2.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{axis}[scale=0.8,axis y line*=left,
            ymin=0, ymax=1,
            xmin=0, xmax=1,
            xmajorgrids,
            xminorgrids,
            xlabel=False Positive Rate,
            ylabel=True Positive Rate,
            	title=U-ROC-Curve $\alpha\equal 1.0$, 
            width=6.5cm, height=5.5cm,
             legend style={at={(1.6,0.5)},anchor=west}, 
            legend style={nodes={scale=0.9, transform shape}}
              ]
\addplot[black, mark=o] coordinates {
(0.0,0.0)
(0.0,0.0017152658662092624)
(0.0,0.008576329331046312)
(0.0,0.010291595197255575)
(0.0,0.015437392795883362)
(0.0,0.018867924528301886)
(0.0,0.032590051457975985)
(0.0,0.0411663807890223)
(0.0,0.058319039451114926)
(0.0,0.0823327615780446)
(0.0,0.09433962264150944)
(0.0,0.1269296740994854)
(0.002398081534772182,0.16123499142367068)
(0.004796163069544364,0.19039451114922812)
(0.007194244604316547,0.21612349914236706)
(0.009592326139088728,0.2469982847341338)
(0.011990407673860911,0.2847341337907376)
(0.016786570743405275,0.32246998284734135)
(0.016786570743405275,0.3567753001715266)
(0.023980815347721823,0.411663807890223)
(0.0407673860911271,0.44768439108061747)
(0.05755395683453238,0.47855917667238423)
(0.08393285371702638,0.5077186963979416)
(0.09112709832134293,0.5540308747855918)
(0.11031175059952038,0.5780445969125214)
(0.1223021582733813,0.6174957118353345)
(0.14388489208633093,0.6380789022298456)
(0.18225419664268586,0.6620926243567753)
(0.2014388489208633,0.6809605488850772)
(0.23261390887290168,0.7186963979416809)
(0.2517985611510791,0.7427101200686106)
(0.2805755395683453,0.7684391080617495)
(0.31894484412470026,0.7873070325900514)
(0.35731414868105515,0.8113207547169812)
(0.39568345323741005,0.8370497427101201)
(0.41007194244604317,0.8576329331046312)
(0.45083932853717024,0.869639794168096)
(0.4892086330935252,0.8902229845626072)
(0.5323741007194245,0.9108061749571184)
(0.565947242206235,0.9262435677530018)
(0.6019184652278178,0.9331046312178388)
(0.6258992805755396,0.9382504288164666)
(0.6666666666666666,0.9536878216123499)
(0.7074340527577938,0.9605488850771869)
(0.7362110311750599,0.9639794168096055)
(0.7889688249400479,0.9691252144082333)
(1.0, 1.0)
    };
    \addlegendentry{Our method};
\addplot[cyan, mark=x] coordinates {
(0.0,0.0)
(0.0,0.0015290519877675841)
(0.0,0.0)
(0.0,0.006144393241167435)
(0.0028735632183908046,0.0015337423312883436)
(0.0,0.0)
(0.0,0.007668711656441718)
(0.0,0.009433962264150943)
(0.0,0.0046875)
(0.0,0.007680491551459293)
(0.002824858757062147,0.01238390092879257)
(0.0028089887640449437,0.010869565217391304)
(0.0028011204481792717,0.013996889580093312)
(0.008771929824561403,0.0182370820668693)
(0.005681818181818182,0.023148148148148147)
(0.0,0.021739130434782608)
(0.003003003003003003,0.026986506746626688)
(0.008849557522123894,0.02723146747352496)
(0.014005602240896359,0.041990668740279936)
(0.008450704225352112,0.037209302325581395)
(0.008620689655172414,0.04754601226993865)
(0.011363636363636364,0.06018518518518518)
(0.028011204481792718,0.05598755832037325)
(0.023121387283236993,0.07033639143730887)
(0.0446927374301676,0.0763239875389408)
(0.04664723032069971,0.0882800608828006)
(0.05014749262536873,0.09682299546142209)
(0.06936416184971098,0.10244648318042814)
(0.07262569832402235,0.14797507788161993)
(0.09798270893371758,0.14088820826952528)
(0.11830985915492957,0.16744186046511628)
(0.12605042016806722,0.16951788491446346)
(0.17796610169491525,0.22445820433436534)
(0.1956521739130435,0.2689873417721519)
(0.3746312684365782,0.3101361573373676)
(0.5116279069767442,0.4054878048780488)
(1.0,1.0)
};
\addlegendentry{MC dropout};

% \addplot[blue, mark=star] coordinates {
% (0.0,0.0)
% (0.0,0.0015923566878980893)
% (0.0,0.0015772870662460567)
% (0.0,0.0015923566878980893)
% (0.0,0.004784688995215311)
% (0.0,0.0031645569620253164)
% (0.0,0.006389776357827476)
% (0.002702702702702703,0.004761904761904762)
% (0.0,0.01594896331738437)
% (0.0027397260273972603,0.006299212598425197)
% (0.0,0.012759170653907496)
% (0.002680965147453083,0.022328548644338118)
% (0.0,0.02527646129541864)
% (0.0,0.01757188498402556)
% (0.0,0.01904761904761905)
% (0.0026595744680851063,0.019230769230769232)
% (0.005361930294906166,0.03189792663476874)
% (0.008241758241758242,0.03930817610062893)
% (0.0027397260273972603,0.04094488188976378)
% (0.013333333333333334,0.0544)
% (0.007978723404255319,0.04807692307692308)
% (0.010899182561307902,0.05845181674565561)
% (0.008021390374331552,0.07987220447284345)
% (0.013774104683195593,0.08006279434850863)
% (0.023809523809523808,0.0932475884244373)
% (0.013333333333333334,0.0864)
% (0.016129032258064516,0.07802547770700637)
% (0.021164021164021163,0.11736334405144695)
% (0.032171581769437,0.11802232854864433)
% (0.03439153439153439,0.12379421221864952)
% (0.03430079155672823,0.13043478260869565)
% (0.02717391304347826,0.13765822784810128)
% (0.06133333333333333,0.1712)
% (0.06318681318681318,0.1918238993710692)
% (0.06824146981627296,0.2035541195476575)
% (0.08042895442359249,0.215311004784689)
% (0.09433962264150944,0.23529411764705882)
% (0.09574468085106383,0.25)
% (0.10723860589812333,0.26953748006379585)
% (0.15447154471544716,0.31695721077654515)
% (0.16939890710382513,0.32018927444794953)
% (0.22282608695652173,0.37183544303797467)
% (0.21680216802168023,0.39619651347068147)
% (0.3007915567282322,0.4428341384863124)
% (0.32075471698113206,0.49920508744038156)
% (0.4666666666666667,0.568)
% (0.5898123324396782,0.6889952153110048)
% (1.0,1.0)
%     };
%     \addlegendentry{MC Dropout, Input = $g(\overline{\mathcal{H}})$};
    
% Evidential Deep Learning

\addplot[orange, mark=|] coordinates {
(0.0,0.0)
(0.0,0.0449438202247191)
(0.006586169045005488,0.23595505617977527)
(0.043907793633369926,0.5056179775280899)
(0.1350164654226125,0.7528089887640449)
(0.24039517014270034,0.8426966292134831)
(0.3358946212952799,0.9213483146067416)
(0.442371020856202,0.9662921348314607)
(0.4983534577387486,0.9662921348314607)
(0.5631174533479693,0.9775280898876404)
(0.6212952799121844,0.9887640449438202)
(0.6761800219538968,1.0)
(0.7135016465422612,1.0)
(0.7530186608122942,1.0)
(0.7793633369923162,1.0)
(0.8079034028540066,1.0)
(0.8320526893523601,1.0)
(0.845225027442371,1.0)
(0.8638858397365532,1.0)
(0.8770581778265643,1.0)
(0.889132821075741,1.0)
(0.8968166849615807,1.0)
(0.9034028540065862,1.0)
(0.9088913282107574,1.0)
(0.9154774972557629,1.0)
(0.9176728869374314,1.0)
(0.9242590559824369,1.0)
(0.9308452250274424,1.0)
(0.9319429198682766,1.0)
(0.9330406147091108,1.0)
(0.9385290889132821,1.0)
(0.9418221734357849,1.0)
(0.9429198682766191,1.0)
(0.9451152579582875,1.0)
(0.9451152579582875,1.0)
(0.9462129527991219,1.0)
(0.9462129527991219,1.0)
(0.9484083424807903,1.0)
(0.9506037321624589,1.0)
(0.9517014270032931,1.0)
(0.9560922063666301,1.0)
(0.9560922063666301,1.0)
(0.9582875960482986,1.0)
(0.960482985729967,1.0)
(0.9626783754116356,1.0)
(0.964873765093304,1.0)
(0.9659714599341384,1.0)
(0.9681668496158068,1.0)
(0.969264544456641,1.0)
(0.969264544456641,1.0)
(0.991218441273326,1.0)
(0.991218441273326,1.0)
(0.991218441273326,1.0)
(0.991218441273326,1.0)
    };
    \addlegendentry{EDL};    
% \addplot[red, mark=asterisk] coordinates {
% (0.0,0.0)
% (0.0,0.010652463382157125)
% (0.0,0.03462050599201065)
% (0.0,0.06524633821571238)
% (0.0,0.13315579227696406)
% (0.0,0.18508655126498003)
% (0.004016064257028112,0.2303595206391478)
% (0.004016064257028112,0.2836218375499334)
% (0.004016064257028112,0.3209054593874834)
% (0.008032128514056224,0.37283621837549935)
% (0.012048192771084338,0.4194407456724368)
% (0.012048192771084338,0.4447403462050599)
% (0.024096385542168676,0.47003994673768307)
% (0.03614457831325301,0.48868175765645805)
% (0.03614457831325301,0.5126498002663116)
% (0.03614457831325301,0.5326231691078562)
% (0.03614457831325301,0.5486018641810919)
% (0.040160642570281124,0.563249001331558)
% (0.040160642570281124,0.5805592543275633)
% (0.04819277108433735,0.5938748335552596)
% (0.0642570281124498,0.6018641810918774)
% (0.07630522088353414,0.6098535286284953)
% (0.08433734939759036,0.6218375499334221)
% (0.08433734939759036,0.6271637816245007)
% (0.09236947791164658,0.6391478029294274)
% (0.09236947791164658,0.6484687083888149)
% (0.10441767068273092,0.6591211717709721)
% (0.12048192771084337,0.6684420772303595)
% (0.1285140562248996,0.6724367509986684)
% (0.13253012048192772,0.6764314247669774)
% (0.13654618473895583,0.6857523302263648)
% (0.13654618473895583,0.6964047936085219)
% (0.14457831325301204,0.7070572569906791)
% (0.1566265060240964,0.7097203728362184)
% (0.1566265060240964,0.7123834886817576)
% (0.1646586345381526,0.7203728362183754)
% (0.17670682730923695,0.7283621837549934)
% (0.18473895582329317,0.729693741677763)
% (0.18875502008032127,0.7310252996005326)
% (0.19678714859437751,0.7350199733688415)
% (0.20883534136546184,0.7416777629826897)
% (0.21285140562248997,0.7443408788282291)
% (0.21285140562248997,0.7456724367509987)
% (0.22088353413654618,0.7470039946737683)
% (0.2289156626506024,0.7509986684420772)
% (0.23694779116465864,0.7509986684420772)
% (0.23694779116465864,0.7536617842876165)
% (0.23694779116465864,0.7549933422103862)
% (0.24096385542168675,0.758988015978695)
% (0.24497991967871485,0.758988015978695)
% (0.25301204819277107,0.758988015978695)
% (0.26104417670682734,0.7616511318242344)
% (0.5020080321285141,0.881491344873502)
% (0.5100401606425703,0.8841544607190412)
% (0.5100401606425703,0.8854860186418109)
% (0.5100401606425703,0.8854860186418109)
% (1.0,1.0)
%     };
%     \addlegendentry{EDL, Input = $g(\overline{\mathcal{H}})$}; 

\addplot[gray,smooth, mark=none, dashed] coordinates {
(0,0)
(1,1)
    };
\addlegendentry{Random}
\end{axis}
\end{tikzpicture}

==> images/figure6/0-01.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}[]
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
            point meta min=-0.3297489971088515,
            point meta max=1.2613392371399446
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp001.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure6/0-1.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
            point meta min=-1.0427578870202487,
            point meta max=1.843386271805002,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp01.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure6/1.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
            point meta min=-3.297489971088515,
            point meta max=3.6839806066935634,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp1.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure6/10.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
            point meta min=-10.51597835991832,
            point meta max=9.504450953344138,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp10.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure6/pipeline.tex <==
\begin{tikzpicture}
  \node[] (0){\input{images/figure6/0-01.tex}};
  \node[above= 0.1cm of 0](0a){$\alpha=0.01$};
  \node[right=0.2cm of 0](1){\input{images/figure6/0-1.tex}};
  \node[above= 0.1cm of 1](1a){$\alpha=0.1$};
  \node[right=0.2cm of 1](2){\input{images/figure6/1.tex}};
    \node[above= 0.1cm of 2](2a){$\alpha=1$};
  \node[right=0.2cm of 2](3){\input{images/figure6/10.tex}};
    \node[above= 0.1cm of 3](3a){$\alpha=10$};
\end{tikzpicture}


==> images/figure8/0-01.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}[]
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=0.0,
point meta max=0.8563167612150242,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp001.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure8/0-1.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=0.0,
point meta max=0.6971393624092874,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp01.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure8/1.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=0.0,
point meta max=0.6000411522012399,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp1.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure8/10.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=0.0,
point meta max=0.49694264048627435,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp10.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure8/pipeline.tex <==
\begin{tikzpicture}
  \node[] (0){\input{images/figure8/0-01.tex}};
  \node[above= 0.1cm of 0](0a){$\gamma=1$};
  \node[right=0.2cm of 0](1){\input{images/figure8/0-1.tex}};
  \node[above= 0.1cm of 1](1a){$\gamma=1.5$};
  \node[right=0.2cm of 1](2){\input{images/figure8/1.tex}};
    \node[above= 0.1cm of 2](2a){$\gamma=2$};
  \node[right=0.2cm of 2](3){\input{images/figure8/10.tex}};
    \node[above= 0.1cm of 3](3a){$\gamma=10$};
\end{tikzpicture}


==> images/figure9/12.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}[]
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=-1.0427578870202487,
point meta max=1.843386271805002,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp12n.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure9/3.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}[]
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=-1.0427578870202487,
point meta max=1.843386271805002,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp03n.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure9/6.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}[]
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=-1.0427578870202487,
point meta max=1.843386271805002,
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp6n.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure9/9.tex <==
\pgfplotsset{colormap/blackwhite,ticks=none}



\begin{tikzpicture}[]
   \begin{axis}[
            width=4cm,
            height=4cm,
            view={0}{90},   % not needed for `matrix plot*' variant
            %
            % added these key-values
            enlargelimits=false,
            axis on top,
point meta min=-1.0849311693251653,
point meta max=1.5482772655797237, 
            %
            % uncomment me to show, that there are really no cells plotted
            % when using the second variant (`surf, shader=flat corner')
            %xmax=5,
            %ymax=5,
        ]
            %% gives the mean temperature of the neighbouring cells (4x4 matrix)
            %\addplot3 [surf] file {temp.dat};

            %% gives the temperature of each point where the reference point
            %% is the lower left corner of the cell (also a 4x4 matrix)
            %% (I already asked the package author if this is intended or a bug)
            %\addplot3 [surf,shader=flat corner] file {temp.dat};

            % this should give the desired output (5x5 matrix)
            \addplot [matrix plot*,point meta=explicit] file {temp9n.dat};
        \end{axis}
\end{tikzpicture}

==> images/figure9/pipeline.tex <==
\begin{tikzpicture}
  \node[] (0){\input{images/figure9/3.tex}};
  \node[above= 0.1cm of 0](0a){$\alpha=0.1, \beta=3$};
  \node[right=0.2cm of 0](1){\input{images/figure9/6.tex}};
  \node[above= 0.1cm of 1](1a){$\alpha=0.1, \beta=6$};
  \node[right=0.2cm of 1](2){\input{images/figure9/9.tex}};
   \node[above= 0.1cm of 2](2a){$\alpha=0.1, \beta=9$};
  \node[right=0.2cm of 2](3){\input{images/figure9/12.tex}};
  \node[above= 0.1cm of 3](3a){$\alpha=0.1, \beta=12$};
\end{tikzpicture}

